Offsets between X-ray and Radio Components in X-ray Jets: The AtlasX

The X-ray emission mechanism of powerful extragalactic jets, which has important implications for their environmental impact, is poorly understood. The X-ray/radio positional offsets in individual features of jets provide important clues. Extending the previous work in Reddy et al. 2021, we present a detailed comparison between X-ray maps deconvolved using the Low Count Image Reconstruction and Analysis (LIRA) tool and radio maps of 164 components from 77 Chandra-detected X-ray jets. We detect 94 offsets (57%), with 58 new detections. In FR II-type jet knots, the X-rays peak and decay before the radio in about half the cases, disagreeing with the predictions of one-zone models. While a similar number of knots lack statistically significant offsets, we argue that projection and distance effects result in offsets below the detection level. Similar de-projected offsets imply that X-rays could be more compact than radio for most knots, and we qualitatively reproduce this finding with a "moving-knot" model. The bulk Lorentz factor derived for knots under this model is consistent with previous radio-based estimates, suggesting kpc-scale jets are only mildly relativistic. An analysis of X-ray/radio flux ratio distributions does not support the commonly invoked mechanism of X-ray production from inverse Compton scattering of the cosmic microwave background but does show a marginally significant trend of declining flux ratio as a function of distance from the core. Our results imply the need for multi-zone models to explain the X-ray emission from powerful jets. We provide an interactive list of our X-ray jet samples at http://astro.umbc.edu/Atlas-X.

==> image_parameters.tex <==
\startlongtable
\begin{deluxetable*}{ccccCc}
  %\centerwidetable
  \tablecaption{Imaging data for the sources discussed in the appendix\label{table:radio-observations}}
  \tabletypesize{\scriptsize}
  \tablehead{
    \colhead{IAU Name} &
    \colhead{Project ID} &
    \colhead{Date}&
    \colhead{Frequency}&
    \colhead{Beam size}&
    \multicolumn{1}{p{2cm}}{\centering X-ray image\\scale}
  }
  \startdata
         0013+790 &             AP0380 &                1999 Aug 02 &        8.4 &    0.25\times0.24 &      log \\
         0017+154 &            15A-357 &                2015 Jun 19 &       14.9 &    0.15\times0.12 &      lin \\
         0034-014 &             AB0534 &                1990 May 25 &        8.4 &    0.35\times0.26 &      log \\
         0035-024 &             AS0179 &                1985 Mar 08 &        4.8 &    0.48\times0.39 &      log \\
         %0055+300 &             AC0476 &                1996 Nov 02 &        4.8 &                   &      lin \\
         0104+321 &             AL0405 &                1996 Nov 13 &        8.4 &    0.24\times0.22 &       lin   \\
         0106+013 &             AR0197 &                1989 Jan 08 &        4.8 &    0.47\times0.39 &      lin \\
         0106+130 &             AR0148 &                1999 Aug 13&        8.4 &      0.22\times0.26 &      log \\
         0133+207 &             AB0796 &                1996 Nov 07 &        4.8 &    0.4\times0.38 &      log \\
          %0206+35 &             AM0221 &                          &            &                   &          \\
         %0208-512 &                    &                          &            &                   &          \\
         0220+427 &             AA0128 &              1991 Aug 19 &        8.4 &    0.24\times0.20 &      lin \\
         0234+285 &             AW0482 &              1998 May 24 &        8.4 &     0.23\times0.22 &      log \\
        % 0313-192 &                    &                          &            &                   &          \\
          0315+41 &             GO0001 &              1993 Feb 23 &        4.8 &      1.4\times1.2 &      lin \\
         0405-113 &             AK0457 &              1998 Apr 30 &        8.4 &      0.36\times0.21&      log \\
          0410+11 &             VG0064 &              1990 Jun 13 &        8.4 &      0.6\times0.45 &      log \\
         % 0413-21 &                    &                          &            &                   &          \\
         0415+379 &             VL0036 &              1985 Apr 07 &        1.4 &    3.41\times2.12 &      log \\
         0430+052 &            16B-353 &              2016 Oct 02 &         10 &    0.22\times0.18 &      lin \\
         0433+295 &             AP0315 &              1995 Aug 07 &        8.4 &    0.22\times0.21 &      lin \\
         %0445+449 &                    &                          &            &                   &          \\
         0454-463 &               C890 (ATCA) &              2000 Sep 03 &       8.64 &2.09\times0.91&      lin \\
          0518-45 &             AR0152 &1987 Oct 27&       14.9 &    0.86\times0.47 &  lin \\
          %0521-36 &                    &                          &            &                   &          \\
         0529+075 &        AH0824 &                   2003 Aug 12 &        4.8 &    0.42\times0.35 &      lin \\
          0605-08 &            16B-332 &              2016 Nov 18 &         10 &    0.26\times0.16 &      log \\
         0637-752 &            C890/6C &              2004 May 09 &       17.1 &0.55\times0.49&      log \\
         0702+749 &             AP0315 &              1995 Aug 06 &        8.4 &    0.40\times0.22 &      lin \\
         0723+679 &             AA0149 &              1992 Nov 10 &        8.4 &    0.29\times0.19 &      log \\
         \multirow{2}{*}{0738+313} &             AG0160 &              1984 Nov 14 &    1.4 &    1.52\times1.29 &  log \\
         &             AG0589 &              2001 Apr 07 &    4.8 &   1.41\times1.22  &  log \\
          %0745+56 &                    &                          &            &                   &          \\
          %0755+37 &                    &                          &            &                   &          \\
         0827+243 &             AM0723 &              2003 Aug 28 &        4.8 &    0.39\times0.38 &      log \\
        0836+2959 &                VAN &              1982 Feb 07 &        4.8 &    0.55\times0.42 &      log \\
         0837+133 &            15A-397 &                2015 Aug 08 &         15 &    0.13\times0.11 &      log \\
          0851+20 &             AS0764 &              2003 Aug 16 &        1.4 &    1.24\times1.13 &      lin \\
         %0855+143 &                    &                          &            &                   &          \\
         %0903-573 &                    &                          &            &                   &          \\
          %0905+39 &                    &                          &            &                   &          \\
         0920-397 &       2016.1.01481 (ALMA) &                          & 97.5 &      0.15\times0.13 &      log \\
          %0917+45 &                    &                          &            &                   &          \\
          0945+07 &       AB0534 &  1989 Apr 07 &    8.4 &    1.18\times0.94 &      log \\
       %             &      AS659 &  1999-jul-10 &    1.4 &    1.18\times0.94 &      log \\
         0957+561 &             AR0247 &              1991 Aug 07 &        8.4 &      0.24\times0.21 &      log \\
         1004+130 &             AW0249 &              1990 May 15 &        8.4 &    0.86\times0.82 &      log \\
         1030-357 &               C890 (ATCA) &              2004 May 12 &         20 &    0.88\times0.47 &      log \\
         1045-188 &             BR0044 &              1996 Dec 13 &        8.4 &    0.5\times0.25  &      log \\
         1046-409 &               C890 (ATCA) & 2004 May 12 &         19 &    0.73\times0.48 &      lin \\
         %1055+201 &                    &                          &        4.8 &                   &          \\
         1111+408 &             AB0522 &              1989 Feb 01 &        4.8 &0.49\times0.37&      log \\
         1055+201 &             BH0025 &              1994 Apr 14 &        8.4 &       0.23\times0.23          &      log \\
         1127-145 &             AC0779 &              2005 May 11 &        8.4 &    0.98\times0.69 &      log \\
         1136-135 &             AH0938 &              2003 Nov 08 &        4.8 &  0.57\times0.55 &      log \\
          1137+660 &             AB0454 &              1987 Jul 12 &        4.8 &  0.53\times0.46 &      log \\
        %1142+1953 &                    &                          &            &                   &          \\
          1142+318 &             AF0186 &                1990 Sep 16 &        8.4 & 0.92\times0.74 &      lin \\
         1150+497 &            16B-189 &                2016 Dec 07 &         15 & 0.12\times0.11 &      log \\
         1202-262 &             AE0059 &                1988 Oct 30 &        4.8 &      0.5\times0.5 &      lin \\
        % 1216+061 &             GP0028 &                          &            &                   &          \\
        1218+339 &             AB0796 &              1996 Nov 12 &        8.4 &    0.22\times0.22 &      log \\
         %1222+216 &             AN0122 &              2004 Oct 06 &        8.4 &                   &      lin \\
         1222+131 &             AW0530 &              2008 Nov 18 &        8.4 &    0.42\times0.41 &      lin \\
          1226+02 &             AT0182 &              1995 Jul 05 &        4.8 &                   &      lin \\
         \multirow{2}{*}{1228+216} &              AO008 &              1990 Apr 25 &        8.4    &    0.31\times0.25 &  lin \\
         &              15A-357 &              2015 Aug 01 &        8.4    &    0.21\times0.19 &  lin \\
          1229-021 &             AK0353 &              1994 Mar 21 &        8.5    & 0.28\times0.26 &      log \\
          1241+26 &             AG0247 &              1987 Sep 14 &        4.8 &    0.42\times0.40 &      log \\
         % 1254+47 &                    &                          &            &                   &          \\
         1305+069 &AB0631&                     1992 Nov 19 &        1.4 &    1.77\times1.30 &     lin     \\
         %1305+069 &                    &                          &        1.4 &                   &          \\
         1317+520 &             AM0723 &              2003 Aug 28 &     4.8       &    0.48\times0.38 &      log \\
         1323+655 &            15A-357 &              2015 Jun 22 &     8.4       &0.20\times0.11&      lin \\
         \multirow{2}{*}{1322-428} & AB0587 &  1991-nov-09 &      8.4      &      2.75\times0.8 &      lin \\
         &             AH0764 &  2002-mar-03 &     8.4       &      0.77\times0.19             &      lin \\
        %        &             AB0587 &  1991-nov-09;2002-mar-03 &            &                   &      lin \\
         1334-127 &             AJ0133 &              1986 Mar 21 &      4.8      &    0.52\times0.59 &      lin \\
         1354+195 &             S71062 &              2006 Feb 06 &        4.8 &    0.47\times0.43 &      lin \\
         1404+344 &              AM024 &              1987 Oct 12 &        4.8 &    0.46\times0.40               &     sqrt \\
         %1409+524 &             AC0238 &              1988 Nov 06 &            &                   &      lin \\
         %1414+110 &             AL0637 &                          &            &                   &          \\
         1421-490 &                    &                          &            &                   &          \\
         1441+522 &             AK0403 &              1995 Jul 27 &        8.4 &    0.41\times0.22 &      lin    \\
         1508+572 &             AM0492 &              1995 Jul 19 &        1.4    &     1.68\times1.21 &      log \\
          1510-089 &             AO0070 &              1986 May 06 &        4.8 &    0.51\times0.39 &      log \\
         %1514-241 &             AB0700 &                          &            &                   &          \\
          %1529+24 &             AV0127 &              1986 Apr 10 &        4.8 &  0.463\times0.351 &      lin \\
         %1547+215 &             AB0755 &                          &            &                   &          \\
         1603+001 &            15A-357 &              2015 Jun 22 &         10 &    0.21\times0.17 &      lin \\
         1600+021 &             AB0534 &              1989 Apr 27 &        8.4 &     0.94\times0.9 &      lin \\
         1609+660 &             AF0231 &              1991 Jul 20 &        4.8 &    0.41\times0.39 &      lin \\
         1637+826 &             VJ0049 & 1988 Nov 20&       1.7     &  1.33\times1.10 &   log       \\
         1641+399 &             AR0196 &              1989 Jan 08 &        8.8 &0.23\times0.22&      log \\
         1641+173 &             AS0179 &              1985 Mar 03 &        4.8 &    0.36\times0.34 &      lin \\
         1642+690 &             AF0310 &              1996 Dec 15 &        8.4 &     0.31\times0.2 &      lin \\
         1704+605 &             UH0001 &              1991 Nov 25 &        8.4 &    1.17\times0.81 &      log \\
         1717+009 &             AS0479 &              1993 Mar 22 &        8.4 &   0.88\times0.83 &      log \\
         1745+624 &            15A-357 &              2015 Jun 22 &         10 &      0.20\times0.16 &      lin \\
         1800+440 &             AD0337 &1994 May 04&        8.4 &    0.24\times0.22 &      lin \\
         1807+698 &             AR0168 &              1988 Nov 25 &        8.4 &     0.34\times0.21 &      lin \\
         %1828+427 &             AW0101 &                          &            &                   &          \\
         1845+797 &             AS0542 &              1994 Nov 28 &        8.4 &      2.73\times2.36 &      lin \\
         1849+670 &            16B-386 &                2016 Sep 08 &         10 &    0.77\times0.55 &      lin \\
         1928+738 &             AE0027 &                1983 Nov 01 &    4.8;1.4 &    0.47\times0.38 &      log \\
         1949+023 &             AB0534 &              1989 Apr 07 &        8.4 &       1.00\times0.98 &      log \\
         1957+405 &             AC0244 &              1989 Jan 06 &        8.4 &          0.25\times0.22 &      lin \\
         2007+777 &             AH0386 &              1990 Mar 27 &        1.4 &    1.57\times1.29 &      log \\
         2043+749 &             AR0386 &                          &        1.4 &                   &          \\
         2104-490 &           2000-may &                          &            &                   &          \\
         2104+463 &             AC0379 &              1994 Jul 02 &        8.4 &0.22\times0.21&      lin \\
         2123-463 &                    &                          &            &                   &          \\
         2152-699 &              C2034 (ATCA) & 2013 Oct 30 &         18.1 &    0.55\times0.47 &          \\
         2155-152 &             AG0499 &              1996 Oct 30 &        8.4 &0.34\times0.23&      log \\
         %2155-152 &                    &                          &        8.4 &                   &          \\
         %2155-152 &                    &                          &        8.4 &                   &          \\
         %2201+315 &             AH1000 &                      &            &                   &          \\
         2201+044 &             AC0641 &              2002 May 08 &       22.5 &    0.27\times0.15 &      lin \\
         2209+080 &             VH0225 &              1986 Jun 01 &        4.8 &    0.45\times0.41 &      lin \\
         2216-038 &            16B-121 &              2016 Nov 01 &          6.0 &    0.43\times0.27 &      log \\
          2221-02 &             AM0772 &              2003 Jul 19 &        8.4 &    0.26\times0.22 &      log \\
         2243+394 &             AB0534 &              1989 Jul 02 &        8.4 &    0.25\times0.25 &      lin \\
         2251+158 &             BR0080 &               2002 Apr 4 &        8.4 &    0.25\times0.23 &      lin \\
         %2255-282 &                    &                          &            &                   &          \\
     %PKSJ2310-437 &                    &                          &            &                   &          \\
          2335+267 &             AH0717 &              2001 Jan 16 &        8.4 &   0.22\times0.21 &      lin \\
         0954+556 &             AM0672 &              2000 Nov 05 &        8.4 &     0.40\times0.21 &      log \\
         %1448+634 &             AH0982 &                     2009 &            &                   &          \\
         1622+158 &             AH0171 &              1985 Jan 02 &        4.8 &     0.48\times0.4 &      lin \\
         % 0651+54 &             AP0315 &              1995 Aug 06 &            &                   &          \\
        0404+035 &             AB0534 &              1990 May 25 &        8.4 &0.25\times0.25&      lin \\
         %1350+316 &             AT0249 &                     2000 &            &                   &          \\
         0459+252 &             AL0164 &                     1987 Oct 09 &     4.8       &    0.39\times0.36 &    lin      \\
         0858+292 &             AS0179 &              1987 Oct 09 &            &                   &      lin \\
         %2247+313 &             BT0018 &              1995 Oct 08 &            &                   &      lin \\
         1251+278 &               VANB &              1981 Mar 18 &      4.8      &    0.44\times0.43 &      lin \\
         1428+422 &             AC0755 &              2004 Dec 06 &      1.4      &    1.82\times1.39 &      log \\
         0031+391 &             AC0200 &                     1987 Oct 06 &            &    0.39\times0.37 &      lin \\
         %0035+130 &                    &                          &            &                   &          \\
         %0038+328 &                    &                          &            &                   &          \\
         0055+016 &             AC0445 & 1995 Dec 02 & &       2.00\times1.47 &      lin \\
         %0145+532 &                    &                          &            &                   &          \\
         %0210+860 &             AH0291 &                19878 Oct 11 &            &                   &      log \\
         %0220+397 &                    &                          &            &                   &          \\
         % 0231+31 &                    &                          &            &                   &          \\
          %0305+03 &                    &                          &            &                   &          \\
         0325+023 &              AP077 &                     1984 Apr 22 &        4.8 &    4.83\times4.29 &      lin\\
         %0725+147 &                    &                          &            &                   &          \\
         0802+013 &             AB1093 &              2004 Sep 08 &     8.4 & 0.26\times0.25 &      log \\
          %0824+29 &             AP0331 &                     1997 &            &                   &      lin \\
         %0855+280 &                    &                          &            &                   &          \\
         %0903+169 &                    &                          &            &                   &          \\
         0947+145 &             AP0331 &                     1996 Dec 15 &        8.4 &0.25\times0.22&      log \\
        % 1157+732 &             AP0380 &              2000 Feb 02 &            &    0.87\times0.62 &      lin \\
         % 1158+31 &                    &                          &            &                   &          \\
         1330+022 &             AS0179 &                     1984 Jan 31 &       4.8     &    2.38\times1.25 &      log \\
         1419+419 &             AP0158 & 1989 Jan 21 &        4.8 &    0.42\times0.35 &      lin \\
          %1508+08 &             AH0452 &                     1991 &            &                   &      lin \\
         1549+628 &             AF0213 &              1991 Jul 20 &        4.8 &     0.4\times0.38 &      lin \\
         1602+014 &             AM9548 & 1996 Oct 26 &        4.8 &         0.41\times0.38          &      lin \\
         1618+177 &             AB0369 &              1986 May 05 &        4.8 & 0.40\times0.38 &     log  \\
         %1626+738 &                    &                          &            &                   &          \\
         %1658+371 &             AL0146 &                     1987 &            &                   &      log \\
         %1802+110 &                    &                          &            &                   &          \\
         %1940+504 &                    &                          &            &                   &          \\
         %2141+279 &             AP0924 &                     1994 &            &                   &      lin \\
        %2145+151  &                    &                          &            &                   &          \\
         %2310+050 &                    &                          &            &                   &          \\
         %2356+437 &                    &                          &            &                   &          \\
         0730+257 &             AK0353 & 1994 Mar 21 &        8.4 &      0.30\times0.21             &      lin \\
         0805+046 &            AH0480        &                     1992 Dec 06 &        8.4 & 0.26\times0.23           &      lin \\
         1311-270 &             AK0353 &              1994 Mar 21 &         8.4   &    0.44\times0.23 &      log \\
         1318+113 &             AK0353 &              1994 Mar 21 &        8.4 &    0.30\times0.23 &      lin \\
         0833+585 &             AL0164 &              1987 Oct 09 &        4.8 &    0.43\times0.38 &      lin \\
         %1834+612 &                    &                          &            &                   &          \\
         %1508+572 &             AM0592 &                     1995 &        1.4 &    1.68\times1.21 &      lin \\
         1343-601 &               C890 (ATCA) &              2002 Feb 02 &      8.6      &    1.35\times1.28 &      log \\
         %1239+376 &                    &                          &            &                   &          \\
         %1418-064 &                    &                          &            &                   &          \\
         0927+362 &             AK0403 &              1995 Jul 27 &        8.4 &0.33\times0.23&     lin     \\
         0610+260 &             VB0072 & 1986 Jun 09 &       5.0     &        0.40\times0.37 &  lin        \\
         \enddata
        \end{deluxetable*}
    

==> list_of_excluded_sources.tex <==
\startlongtable
\begin{longrotatetable}
\begin{deluxetable*}{ccccchccc}
  %\centerwidetable

  \tablecaption{List of \textit{Chandra} detected X-ray jets excluded from offset analysis\label{table:list_of_excluded_sources}}
  \tabletypesize{\scriptsize}
  \tablehead{
    \colhead{ Name} &
    \colhead{IAU Name} &
    \multicolumn{1}{p{2cm}}{\centering R.A. (J2000)\\hh:mm:ss} &
    \multicolumn{1}{p{2cm}}{\centering decl. (J2000)\\dd:mm:ss} &
    \colhead{z} &
    \nocolhead{$D_L$} &
    \multicolumn{1}{p{2cm}}{\centering kpc Scale\textsuperscript{c}\\(kpc/arcsec) } &
    \colhead{Class}&
    \multicolumn{1}{p{3cm}}{\centering Detection\\paper }
  }
  \tablecolumns{9}
  \startdata
  \cutinhead{Jets with FR II morphology}
  3C6.1 & 0013+790 & 00:16:31.147		 & +79:16:49.88	 & 0.8400 & 5342 & 7.84 & FR II (NLRG) &  \citet{2004ApJ...612..729H} \\
  3C13 & 0031+391 & 00:34:14.556 & +39:24:16.65 & 1.351 & 9830 & 8.63 & FR II (NLRG) & \citet{wilkes2013revealing} \\
  3C17 & 0035-024 & 00:38:20.520	 & -02:07:40.72	 & 0.2200 & 1081 & 3.64 & FR II (BLRG) &\citet{Massaro_2009} \\
  4C+28.07 & 0234+285 & 02:37:52.405 & +28:48:08.99	 & 1.2130 & 8445 & 8.36 & CDQ &\citet{marshall2011x}\\
  3C33 & 0106+130 & 01:08:52.860	 & +13:20:13.80	 & 0.0597 & 264 & 1.14 & FR II (NLRG)& \citet{2007ApJ...659.1008K}\\
  3C16 & 0035+130 & 00:37:44.573 & +13:19:54.99 & 0.4050 & 2260 & 5.567 & FR II & \citet{massaro2013chandra}\\
  0529+075 & 0529+075 & 05:32:38.998	 & +07:32:43.34 & 1.2540 & 8803 & 8.40 & CDQ &\citet{2011ApJ...730...92H}\\
  PKS 0637-752 & 0637-752 & 06:35:46.508	 & -75:16:16.81	 & 0.6510 & 3909 & 6.90 & CDQ &\citet{chartas2000chandra}\\
  3C 173.1 & 0702+749 & 07:09:18.124 & +74:49:31.80 & 0.2920 & 1494 & 4.30 & FR II (LERG) &\citet{2004ApJ...612..729H}\\
  4C +55.17 & 0954+556 & 09:57:38.184 & +55:22:57.76 & 0.8996 & 5960 & 8.01 & Q &\citet{tavecchio2007chandra}\\
  3C 273 & 1226+023 & 12:29:06.699	 & +02:03:08.59 & 0.1500 & 749 & 2.70 & CDQ &\citet{marshall2001structure}\\
  PKS 1311-270 & 1311-270 & 13:13:47.360 & -27:16:49.27 & 2.1860 & 18500 & 8.43 & Q &\citet{McKeough_2016}\\
  Cygnus A & 1957+405 & 19:59:28.355	 & +40:44:01.89	 & 0.0560 & 247 & 1.07 & FR II RG &\citet{wilson2000chandra} \\
  1849+670 & 1849+670 & 18:49:16.072	 & +67:05:41.68	 & 0.6570 & 3938 & 6.95 & CDQ &\citet{2011ApJ...730...92H}\\
  4C+62.29 & 1745+624 & 17:46:14.034	 & +62:26:54.74	 & 3.8890 & 35316 & 7.20 & LDQ &\citet{Cheung_2006}\\
  NGC 6251 & 1637+826 & 16:32:31.969 & +82:32:16.39 & 0.0240 & 107 & 0.49 & FRI/II (LERG)&\citet{evans2005chandra} \\
  3C 330 & 1609+660 & 16:09:36.607	 & +65:56:43.61	 & 0.5500 & 3169 & 6.40 & FR II (NLRG) &\citet{2002ApJ...581..948H}\\
  3C 325 & 1549+628 & 15:49:58.420 & +62:41:21.66 & 1.1350 & 7940 & 8.44 & FR II& \citet{salvati2008x}\\
  3C 321 & 1529+242 & 15:31:43.474	 & +24:04:19.02	 & 0.0960 & 435 & 1.80 & FR II (NLRG)& \citet{2004ApJ...612..729H}\\
  TXS 1508+572 & 1508+572 & 15:10:02.923 & +57:02:43.37 & 4.3087 & 40100 & 6.89 & Q&\citet{siemiginowska2003x} \\
  AP Lib & 1514-241 & 15:17:41.813 & -24:22:19.48 & 0.0486 & 213 & 0.94 & BL Lac &\citet{kaufmann2013discovery}\\
  4C+19.44 & 1354+195 & 13:57:04.436 & +19:19:07.37 & 0.7196 & 4410 & 7.20 & CDQ &\citet{sambruna2004survey}\\
  B3 1428+422 & 1428+422 & 14:30:23.741 & +42:04:36.49 & 4.7150 & 44600 & 6.61 &  Q&\citet{Cheung_2012}\\
  4C+11.45 & 1318+113 & 13:21:18.835 & +11:6:49.98 & 2.1792 & 17700 & 8.48 & Q &\citet{McKeough_2016}\\
  4C+65.15 & 1323+655 & 13:25:29.702 & +65:15:13.293 & 1.6250 & 12163 & 8.60 & LDQ &\citet{Miller_2009}\\
  3C 228 & 0947+145 & 09:50:10.791 & +14:20:0.63 & 0.5524 & 3300 & 6.62 & FR II (NLRG) &\citet{2004ApJ...612..729H}\\
  4C+13.41 & 1004+130 & 10:07:26.099	 & +12:48:56.19	 & 0.2400 & 1193 & 3.76 & LDQ &\citet{2006ApJ...652..163M}\\
  PKS 1046-409 & 1046-409 & 10:48:38.270 & -41:14:00.11 & 0.6200 & 3668 & 6.78 & CDQ &\citet{2005ApJS..156...13M}\\
  3C 227 & 0945+076 & 09:47:45.143 & +07:25:20.59 & 0.08610 & 388 & 1.59 & FR II (BLRG) &\citet{2007ApJ...669..893H}\\
  TXS 0833+585 & 0833+585 & 08:37:22.409 & +58:25:1.84 & 2.1010 & 16900 & 8.53 & Q &\citet{McKeough_2016}\\
  3C 179 & 0723+679 & 07:28:10.896 & +67:48:47.03 & 0.8460 & 5386 & 7.70 & LDQ &\citet{sambruna2004survey}\\
  Pictor A & 0518-458 & 05:19:49.690	 & -45:46:44.50	 & 0.0350 & 152 & 0.69 & FR II (BLRG) &\citet{2001ApJ...547..740W}\\
  3C19 & 0038+328 & 0:40:55.0440 & +33:10:8.0200 & 0.4820 & 2780 & 6.15 & FR II (LERG) &\citet{massaro2015chandra}\\
  3C52 & 0145+532 & 01:48:28.977 & +53:32:35.44 & 0.2900 & 1530 & 4.47 &FR II (HERG) &\citet{massaro2010chandra}\\
  3C41 & 0123+239 & 01:26:44.300 & +33:13:11.00 & 0.7950	& 511	 & 7.70	& FR II (HERG)&\citet{Massaro_2018}\\
  3C54 & 0152+435 & 01:55:30.162 & 	+43:45:55.43 & 0.8270 &	537 & 	7.81	& FR II (HERG)&\citet{Massaro_2018}\\
  3C61.1 & 0210+860 & 02:22:35.046 & +86:19:06.17 & 0.1878 & 941.0 & 3.32 &FR II (HERG) &\citet{massaro2010chandra}\\
  3C65 & 0220+397 & 02:23:43.191 & +40:00:52.45 & 1.1760 & 8290 & 8.49 &FR II (HERG) &\citet{wilkes2013revealing}\\
  3C68.2 & 0231+313 & 02:34:23.856 & +31:34:17.46 & 1.5750 & 11900 & 8.69 & FR II (HERG)&\citet{wilkes2013revealing}\\
  3C105 & 0404+0333 & 04:07:16.480 & +03:42:25.81 & 0.0890 & 418 & 1.71 & FR II&\citet{massaro2010chandra}\\
  3C109 & 0410+110 & 04:13:40.343 & +11:12:13.79 & 0.3056 & 1574 & 4.50 & FR II (BLRG) &\citet{2004ApJ...612..729H}\\
  PKS0413-21 & 0413-210 & 04:16:04.359 & -20:56:27.51 & 0.8080 & 5087 & 7.54 & CDQ&\citet{2005ApJS..156...13M}\\
  3C154\tablenotemark{*} & 0610+260 & 06:13:50.139	& +26:04:36.71	& 0.5800	& 349	& 6.77	& Q&\citet{Massaro_2018}\\
  3C171 & 0651+542 & 06:55:14.809 & +54:09:00.15 & 0.2384 & 1230& 3.89 & FR II (HERG)&\citet{massaro2010chandra}\\
  3C181 & 0725+147 & 07:28:10.305 & 14:37:36.24 & 1.3820 & 10100 & 8.64 & Q&\citet{wilkes2013revealing}\\
  4C+25.21 & 0730+257 & 07:33:08.784 & +25:36:25.06 & 2.6860 & 22800 & 8.13& Q&\citet{McKeough_2016}\\
  %DA240 & 0745+560 & 07:48:37.900 & +55:48:58.00 & 0.0357 & 155.0 & 0.70 & FRII RG&\citet{}\\
  3C191 & 0802+013 & 08:04:47.972 & 10:15:23.69 & 1.9560 & 15500 & 8.60 & Q&\citet{erlund2006extended}\\
  4C +05.34 & 0805+046 & 08:07:57.538 & +04:32:34.53 & 2.8770 & 24800 & 7.98 & Q&\citet{McKeough_2016}\\
  3C200 & 0824+294 & 08:27:25.397 & +29:18:44.90 & 0.4580 & 2630 & 5.99 & FR II (LERG)&\citet{2004ApJ...612..729H}\\
  3C210 & 0855+280 & 08:58:09.961 & +27:50:51.57 & 1.1690 & 8240 & 8.48 & FR II (HERG)&\citet{gilmour2009distribution}\\
  3C212 & 0855+143 & 08:58:41.447 & +14:09:44.77 & 1.049 & 7043 & 8.10 & LDQ&\citet{2003ApJ...597..751A}\\
  3C213.1 & 0858+292 & 09:01:05.251 & +29:01:46.90 & 0.194 & 981.0 & 3.33 & FR II (LERG) & \citet{massaro2010chandra}\\
  PKS0903-573 & 0903-573 & 09:04:53.179 & -57:35:05.80 & 0.6950 & 4221 & 7.12 & CDQ&\citet{2005ApJS..156...13M}\\
  %3C215 & 0903+169 & 09:06:31.873 & +16:46:11.87 & 0.4121 & 2320 & 5.64 & Q&\citet{2004ApJ...612..729H}\\
  4C+39.24 & 0905+399 & 09:08:16.900 & +39:43:26.00 & 1.882 & 14800 & 8.63 & FR II (HERG)&\citet{2008MNRAS.386.1774E}\\
  3C219 & 0917+458 & 09:21:08.626 & +45:38:57.34 & 0.1740 & 831 & 2.90& FR II RG (HERG)&\citet{2003MNRAS.340L..52C}\\
  2155-152 & 2155-152 & 21:58:06.282	 & -15:01:09.32	 & 0.6720 & 4049 & 7.02 & CDQ &\citet{2011ApJ...730...92H}\\
  4C+74.26 & 2043+749 & 20:42:37.308 & +75:08:02.45 & 0.1040 & 474 & 1.90 & LDQ &\citet{erlund2007luminous}\\
  3C 445 & 2221-020 & 22:23:49.530 & -02:06:12.85 & 0.0560 & 247 & 1.10 & FR II RG &\citet{Perlman_2009}\\
  %3c220.2 & 0927+362 & 09:30:33.473 &	+36:01:24.17 &	1.1574	& 814	& 8.47	& Q&\citet{Stuardi_2018}\\
  3C225B & 0939+139 & 09:42:15.387& 	+13:45:50.52 & 	0.5800 & 	349	 & 6.77 & 	FR II (HERG)&\citet{Massaro_2018}\\
  3C238 & 1008+066 & 10:11:00.379 &	+06:24:39.72 & 	1.4050	 & 10300 & 	8.65	 & FR II (HERG)&\citet{Stuardi_2018}\\
  3C268.1 & 1157+732 & 12:0:19.210 & +73:00:45.70 & 0.9700 & 6540 & 8.17 & FR II (NLRG)&\citet{massaro2015chandra} \\
  3C268.2 & 1158+318 & 12:00:59.110 & +31:33:27.90 & 0.3620 & 2000 & 5.21 & FR II (HERG) &\citet{massaro2012chandra}\\
  %B3 1239+376 & 1239+376 & 12:42:09.812 & +37:20:5.69 & 3.8190 & 34800 & 7.25 & &\citet{}\\
  3C280 & 1254+476 & 12:56:57.900 & +47:20:19.90 & 0.9960 & 6601 & 8.00 & FR II (HERG)&\citet{donahue2003constraints}\\
  3C281 & 1305+069 & 13:07:53.929 & +06:42:14.30 & 0.6020 & 3538 & 6.70 & LDQ&\citet{crawford2003extended}\\
  3C295 & 1409+524 & 14:11:20.647	 & +52:12:09.04	 & 0.4500 & 2486 & 5.70 & FR II (NLRG) &\citet{massaro2013chandra}\\
  3C297 & 1414-037 & 14:17:23.999	&-04:00:47.54 & 	1.4061 & 	10300 & 	8.65 & 	Q&\citet{Stuardi_2018}\\
  PKS 1418-064 & 1418-064 & 14:21:07.755 & -06:43:56.35 & 3.6890 & 33400 & 7.35 & Q&\citet{McKeough_2016}\\
  PKS1421-490 & 1421-490 & 14:24:32.237 & -49:13:49.74 & 0.6620 & 3978.6 & 6.98 & Q&\citet{gelbord2005knotty}\\
  %3C305 & 1448+634 & 14:49:21.573 & +63:16:13.97 & 0.0416 & 191 & 0.85 & FRII & \\
  3C313 & 1508+080 & 15:11:00.010 & +07:51:50.00 & 0.4610 & 2650 & 6.01 & FR II (HERG)&\citet{massaro2013chandra}\\
  3C324 & 1547+215 & 15:49:48.900 & +21:25:38.10 & 1.2063 & 8387 & 8.40 & FR II (HERG)&\citet{2004ApJ...612..729H}\\
  3C327.1\tablenotemark{*} & 1602+014 & 16:04:45.320 & +01:17:51.02& 0.4620 & 2660 & 6.02 & FR II (HERG)&\citet{massaro2013chandra}\\
  3C341 & 1626+738 & 16:28:4.050 & +27:41:43.00 & 0.4480 & 2560 & 5.91 & FR II (HERG) & \citet{massaro2013chandra}\\
  3C349 & 1658+371 & 16:59:29.540 & +47:02:44.10 & 0.2050 & 1040 & 3.46 & FR II (HERG)&\citet{massaro2010chandra}\\
  %3C368 & 1802+110 & 18:05:06.454 & 11:01:35.060 & 1.1310 & 7900 & 8.44 & FR II (HERG)&\citet{}\\
  3C 380 & 1828+427 & 18:29:03.781 & +48:44:46.60 & 0.6920 & 4199 & 7.11 & CDQ &\citet{marshall2005chandra}\\
  TXS1834+612 & 1834+612 & 18:35:19.675 & +61:19:40.01 & 2.2740 & 18600 & 8.42 & Q&\citet{McKeough_2016}\\
  3C402 & 1940+504 & 19:41:46.050 & +50:35:48.40 & 0.0259 & 114 & 0.53 & FR I&\citet{massaro2012chandra}\\
  PKS2101-49 & 2104-490 & 21:05:01.157 & -48:48:46.52 & 1.0400 & 6967 & 8.12 & CDQ&\citet{marshall2005chandra}\\
  2123-463 & 2123-463 & 21:26:30.704 & -46:05:47.90 & 1.6700 & 12583 & 8.56 & CDQ&\citet{marshall2011x}\\
  3C436 & 2141+279 & 21:44:11.708 & +28:10:19.03 & 0.2145 & 1090 & 3.57 & FR II (HERG)&\citet{massaro2010chandra}\\
  3C437 & 2145+151 & 21:47:25.106 & +15:20:37.49 & 1.4800 & 11000 & 8.68 & FR II&\citet{massaro2015chandra}\\
  PKS2152-69 & 2152-699 & 21:57:05.977 & -69:41:23.68 & 0.0283 & 122 & 0.56 & FR II RG&\citet{ly2005discovery}\\
  4C+31.63 & 2201+315 & 22:03:14.975 & +31:45:38.30 & 0.2950 & 1511 & 4.37 & CDQ&\citet{2011ApJ...730...92H}\\
  2255-282 & 2255-282 & 22:58:05.962 & -27:58:21.30 & 0.9260 & 6027 & 7.88 & CDQ&\citet{marshall2011x}\\
  3C458 & 2310+050 & 23:12:54.408 & +05:16:45.98 & 0.2890 & 1530 & 4.46 & FR II (HERG)&\citet{massaro2012chandra}\\
  3C470 & 2356+437 & 23:58:35.890 & +44:4:45.55 & 1.653. & 12600 & 8.69 & FR II&\citet{2011ApJ...730...92H}\\
  \cutinhead{Jets with FR I morphology}
  3C 29 & 0055+016 & 00:57:34.916 & -01:23:27.92 & 0.0450 & 201 & 0.89 & FR I (LERG) &\citet{massaro2012chandra}\\
  NGC315 & 0055+300 & 00:57:48.883 & +30:21:08.81& 0.0165 & 70.6 & 0.32 & FR I RG &\citet{worrall2003x}\\
  4C+35.03 & 0206+355 & 02:09:38.560 & +35:47:50.90 & 0.0369 & 160 & 0.72 & FR I RG&\citet{worrall2001chandra}\\
  3C78 & 0305+039 & 03:08:26.223 & +04:06:39.30 & 0.0286 & 127 & 0.58 & FR I (LERG) &\citet{harwood2012determines}\\
  0313-192 & 0313-192 & 03:15:52.100 & -19:06:44.30 & 0.0670 & 298 & 1.27 & FR I RG&\citet{2006AJ....132.2233K}\\
  3C129 & 0445+449 & 04:49:09.064 & +45:00:39.40 & 0.0208 & 89 & 0.42 & FR I RG&\citet{harris2002c}\\
  PKS0521-36 & 0521-365 & 05:22:57.983 & -36:27:30.80 & 0.0550 & 242 & 1.06 & BL Lac&\citet{birkinshaw2002x}\\ 
  3C 346 & 1641+173 & 16:43:48.605 & +17:15:49.43 & 0.1610 & 762.6 & 2.74 & FRI (NLRG) &\citet{2005MNRAS.360..926W}\\
  CenA & 1322-428 & 13:25:27.615 & -43:01:08.80 & 0.0018 & 3.8 & 0.02 & FRI RG &\citet{kraft2000chandra}\\
  CenB & 1343-601 & 13:46:48.990 & -60:24:29.96 & 0.0130 & 55.5 & 0.26 & FRI RG &\citet{2005ApJS..156...13M}\\
  3C189 & 0755+379 & 07:58:28.108 & +37:47:11.80& 0.0428 & 187.0 & 0.83 & FR I RG&\citet{worrall2001chandra}\\
  3C264 & 1142+195 & 11:45:05.009 & +19:36:22.70 & 0.0217 & 93.0 & 0.43 & FR I (LERG)&\citet{2010ApJ...708..171P}\\
  NGC4261 & 1216+061 & 12:19:23.216 & +05:49:30.80 & 0.0073 & 31 & 0.15 & FR I RG&\citet{chiaberge2003hubble}\\
  3C293 & 1350+316 & 13:52:17.842& +31:26:46.50 & 0.0450 & 209 & 0.92 & FR I (LERG) &\citet{massaro2010chandra}\\
  3C296 & 1414+110 & 14:16:52.928 & +10:48:27.70 & 0.0237 & 102 & 0.47 & FR I (LERG)&\citet{hardcastle2005chandrab}\\
  NGC7385 & 2247+113 & 22:49:54.586 & +11:36:30.84 & 0.0280 & 112000 & 0.52 & FR I&\citet{rawes2015discovery}\\
  PKSJ2310-437 & 2310-437 & 23:10:43.600 & -43:47:34.30 & 0.0886 & 400 & 1.60 & FR I RG&\citet{2009ApJ...698.1061B}\\
  \enddata
  \tablecomments{Same as Table \ref{table:list_of_sources} but with the sources that are excluded from the offset analysis} 
 %\tablecomments{Comments place holder}
%\tablenotetext{a}{test footnote}
%% General table references marker
%\tablerefs{\ref{test}}
\end{deluxetable*}
\end{longrotatetable}


==> list_of_sources.tex <==
\startlongtable
%\begin{longrotatetable}
\begin{deluxetable*}{lchhchcll}
  %\centerwidetable

  \tablecaption{List of \textit{Chandra} detected X-ray jets considered for offset analysis\label{table:list_of_sources}}
  \tabletypesize{\scriptsize}
  \tablehead{
    \colhead{Name\textsuperscript{a}} &
    \colhead{IAU Name\textsuperscript{b}} &
    %\multicolumn{1}{p{2cm}}{\centering R.A. (J2000)\textsuperscript{c}\\hh:mm:ss} &
    %\multicolumn{1}{p{2cm}}{\centering decl. (J2000)\textsuperscript{c}\\dd:mm:ss} &
    \nocolhead{ra}&
    \nocolhead{dec}&
    \colhead{z\textsuperscript{c}} &
    \nocolhead{$D_L$} &
    %\colhead{kpc/arcsec}&
    %\multicolumn{1}{p{2cm}}{\centering kpc Scale\textsuperscript{c}\\(kpc/arcsec) } &
    \colhead{kpc/arcsec\textsuperscript{d}}&
    \colhead{Class\textsuperscript{e}}&
    \colhead{Reference\textsuperscript{f}}
    %\multicolumn{1}{p{3cm}}{\centering Detection\textsuperscript{f}\\paper }
  }
  \tablecolumns{9}
  \startdata
  \cutinhead{Jets with FR-II type morphology}
  3C 9 & 0017+154 & 00:20:25.220	 & +15:40:54.73	 & 2.012  & 15850 & 8.57 & LDQ & \citet{2003MNRAS.338L...7F}\\
  4C+01.02 & 0106+013 & 01:08:38.770	 & +01:35:0.31 & 2.099 & 16702 & 8.43 & CDQ &\citet{2011ApJ...730...92H}\\
  3C 47 & 0133+207 & 01:36:24.423	 & +20:57:27.40	 & 0.4250 & 2322 & 5.50 & LDQ &\citet{2004ApJ...612..729H}\\
  PKS 0208-512 & 0208-512 & 02:10:46.200 & -51:01:01.89 & 0.9990 & 6626.0 & 8.04 & CDQ&\citet{2005ApJS..156...13M}\\
  PKS 0405-12 & 0405-113 & 04:07:48.430	 & -12:11:36.60 & 0.5740 & 3338 & 6.50 & CDQ &\citet{sambruna2004survey}\\
  3C 109 & 0410+110 & 04:13:40.343 & +11:12:13.79 & 0.3056 & 1574 & 4.50 & FR II (BLRG) &\citet{2004ApJ...612..729H}\\
  3C 111 & 0415+379 & 04:18:21.277 & +38:01:35.80 & 0.0491 & 215 & 0.95 & FR II (BLRG) &\citet{2011ApJ...730...92H}\\
  3C 123 & 0433+295 & 04:37:04.367	 & +29:40:13.67	 & 0.2177 & 1068 & 3.49 & FR II (LERG) &\citet{hardcastle2001chandra}\\
  PKS 0454-46 & 0454-463 & 04:55:50.772 & -46:15:58.68 & 0.8580 & 5481 & 7.70 & CDQ &\citet{marshall2011x}\\
  3C 133 & 0459+252 & 05:02:58.480 & +25:16:25.11 & 0.2775 & 1460 & 4.34 & FR II (HERG) &\citet{massaro2010chandra}\\
  PKS 0605-08 & 0605-085 & 06:07:59.699	 & -08:34:49.97 & 0.8700 & 5577 & 7.70 & CDQ &\citet{sambruna2004survey}\\
  B2 0738+313 & 0738+313 & 07:41:10.703 & +31:12:00.23 & 0.6310 & 3777 & 6.90 & CDQ& \citet{siemiginowska2003chandra}\\
  0827+243 & 0827+243 & 08:30:52.086	 & +24:10:59.82	 & 0.9390 & 6133 & 7.90 & CDQ &\citet{2004ApJ...614..615J}\\
  4C+29.30 & 0836+299 & 08:40:02.279	 & +29:49:00.47	 & 0.0640 & 284 & 1.20 & FRI RG &\citet{sambruna2004survey}\\
  3C 207 & 0837+133 & 08:40:47.588 & +13:12:23.56 & 0.6800 & 4109 & 7.10 & LDQ &\citet{2002AA...381..795B}\\
  PKS 0920-397 & 0920-397 & 09:22:46.413	 & -39:59:34.96	 & 1.8800 & 14574 & 8.50 & CDQ &\citet{2005ApJS..156...13M} \\
  QSO B0957+561 & 0957+561 & 10:01:20.990	 & +55:53:56.52	 & 1.4100 & 10191 & 8.50 & LDQ &\citet{chartas2002constraining}\\
  PKS 1030-357 & 1030-357 & 10:33:07.660	 & -36:01:56.80	 & 1.4550 & 10599 & 8.53 & CDQ &\citet{2005ApJS..156...13M}\\
  PKS 1045-188 & 1045-188 & 10:48:06.621	 & -19:09:35.72	 & 0.5950 & 3487 & 6.64 & CDQ &\citet{2011ApJ...730...92H}\\
  PKS 1055+201 & 1055+201 & 10:58:17.900 & +19:51:50.87 & 1.1100 & 7558 & 8.20 & LDQ &\citet{schwartz2006discovery}\\
  3C 254 & 1111+408 & 11:14:38.482	 & +40:37:20.28	 & 0.7340 & 4516 & 7.30 & LDQ &\citet{donahue2003constraints}\\
  PKS 1127-145 & 1127-145 & 11:30:07.051	 & -14:49:27.41	 & 1.1800 & 8159 & 8.30 & CDQ &\citet{siemiginowska2002chandra}\\
  PKS 1136-135 & 1136-135 & 11:39:10.702 & -13:50:43.63 & 0.5540 & 3197 & 6.40 & LDQ &\citet{sambruna2002survey}\\
  3C 263 & 1137+660 & 11:39:57.039	 & +65:47:49.40 & 0.6563 & 3934 & 7.00 & LDQ &\citet{2002ApJ...581..948H}\\
  3C 265 & 1142+318 & 11:45:28.911 & +65:47:49.43 & 0.8110 & 5110 & 7.55 & FR II (NLRG) &\citet{2004MNRAS.354L..43B}\\
  4C+49.22 & 1150+497 & 11:53:24.407	 & +49:31:06.95	 & 0.3340 & 1746 & 4.80 & CDQ &\citet{sambruna2002survey}\\
  PKS 1202-262 & 1202-262 & 12:05:33.210	 & -26:34:04.46 & 0.7890 & 4939 & 7.48 & CDQ &\citet{2005ApJS..156...13M}\\
  3C 270.1 & 1218+339 & 12:20:33.875 & +33:43:12.03 & 1.528 & 11500 & 8.69 & Q &\citet{2012ApJ...745...84W} \\
  4C+21.35 & 1222+216	 & 21:22:46.380	 & +21:22:46.40 & 0.4320 & 2367 & 5.60 & CDQ &\citet{jorstad2006x}\\
  PKS 1229-02 & 1229-021 & 12:32:00.010	 & -02:24:05.30 & 1.0450 & 7009 & 8.10 & CDQ &\citet{tavecchio2007chandra}\\
  3C275.1 & 1241+266 & 12:43:57.649 & +16:22:53.39 & 0.5550 & 3204 & 6.40 & LDQ &\citet{crawford2003extended}\\
  3C 277.3 & 1251+278 & 12:54:12.052 & +27:37:33.95 & 0.0853 & 406 & 1.66 & FR II (HERG) &\citet{worrall2016x}\\
  4C+52.27 & 1317+520 & 13:19:46.190 & +51:48:05.79 & 1.0600 & 7135 & 8.15 & CDQ&\citet{jorstad2006x} \\
  3C 287.1 & 1330+022 & 13:32:53.270 & +02:00:45.69 & 0.2155 &  & 3.619 & FR II (BLRG) &\citet{balmaverde2012extended}\\
  PKS 1334-127 & 1334-127 & 13:37:39.782 & -12:57:24.69 & 0.5390 & 3091 & 6.33 & CDQ &\citet{2011ApJ...730...92H}\\
  3C 294 & 1404+344 & 14:06:44.022	 & +34:11:25.10	 & 1.7860 & 13677 & 8.50 & FR II (NLRG) &\citet{2003MNRAS.341..729F}\\
  3C 299 & 1419+419 & 14:21:05.696 & +41:44:48.50 & 0.3670 & 2030 & 5.25 & FR II (NLRG) &\citet{massaro2010chandra}\\
  3C 303 & 1441+522 & 14:43:02.777	 & +52:01:37.33	 & 0.1410 & 659 & 2.50 & FR II (BLRG) &\citet{kataoka2003chandra}\\
  PKS 1510-08 & 1510-089 & 15:12:50.536	 & -09:05:59.73	 & 0.3610 & 1913 & 5.00 & CDQ &\citet{sambruna2004survey}\\
  3C 325 & 1549+628 & 15:49:58.420 & +62:41:21.66 & 1.1350 & 7940 & 8.44 & FR II& \citet{salvati2008x}\\
  4C+00.58 & 1603+001 & 16:06:12.683 & +00:00:27.21 & 0.0590 & 261 & 1.10 & LDQ &\citet{2010ApJ...717L..37H}\\
  3C334 & 1618+177 & 16:20:21.818 & +17:36:2.95 & 0.5551 & 3310 & 6.63 & Q &\citet{2004ApJ...612..729H}\\
  4C+15.55 & 1622+158 & 16:25:14.373 & +15:45:21.94 & 1.4060 & 10300 & 8.65 & FR II &\citet{stockton2006extremely}\\
  4C+69.21 & 1642+690 & 16:42:07.849	 & +68:56:39.7	 & 0.7510 & 4646 & 7.30 & CDQ &\citet{sambruna2004survey}\\
  3C 345 & 1641+399 & 16:42:58.810	 & +39:48:37.00	& 0.5940 & 3481 & 6.60 & CDQ &\citet{sambruna2004survey}\\
  3C 351 & 1704+605 & 17:04:41.417	 & +60:44:30.65	 & 0.3720 & 1982 & 5.10 & LDQ &\citet{2001ApJ...561L.157B}\\
  TXS 1800+440 & 1800+440 & 18:01:32.315	 & +44:04:21.90 & 0.6630 & 3983 & 6.98 & CDQ &\citet{2011ApJ...730...92H}\\
  3C 380 & 1828+427 & 18:29:03.781 & +48:44:46.60 & 0.6920 & 4199 & 7.11 & CDQ &\citet{marshall2005chandra}
  3C 390.3 & 1845+797 & 18:42:08.981	 & +79:46:17.21	 & 0.0561 & 247 & 1.08 & FR II (BLRG) &\citet{2007ApJ...669..893H}\\
  4C +73.18 & 1928+738 & 19:27:48.500 & +73:58:01.60 & 0.3020 & 1553 & 4.40 & CDQ &\citet{sambruna2004survey}\\
  3C 403 & 1949+023 & 19:52:15.796	 & +02:30:24.39 & 0.0590 & 260.6 & 1.12 & FR II (NLRG) &\citet{2005ApJ...622..149K}\\
  4C +08.64 & 2209+080 & 22:12:01.589	 & +08:19:16.51	 & 0.4850 & 2721 & 5.98 & CDQ &\citet{jorstad2006x}\\
  4C -03.79 & 2216-038 & 22:18:52.038	 & -03:35:36.88	 & 0.9010 & 5825 & 7.81 & (FRI/II) CDQ &\citet{2011ApJ...730...92H}\\
  3C 452 & 2243+394 & 22:45:48.770	 & +39:41:15.70 & 0.0811 & 364 & 1.50 & FR II (NLRG) &\citet{2004ApJ...612..729H}\\
  3C454.3 & 2251+158 & 22:53:57.750	 & +16:08:53.56 & 0.8590 & 5489 & 7.70 & CDQ &\citet{2005ApJS..156...13M}\\
  \cutinhead{Jets with FR-I type morphology}
  3C 15 & 0034-014 & 00:37:04.114	 & -01:09:08.46	 & 0.0730 & 326 & 1.40 & FRI (NLRG)&\citet{2003AA...410..833K} \\
  3C 31 & 0104+321 & 01:07:24.961	 & +32:25:45.01	 & 0.0167 & 71.4 & 0.34 & FRI (LERG) &\citet{hardcastle2002chandra} \\
  4C+35.03 & 0206+355 & 02:09:38.531 & +35:47:51.08 & 0.0377 & 168 & 0.72 & FR I (RG) & \citet{2001MNRAS.326L...7W} \\
  3C66B & 0220+427 & 02:23:11.409	 & +43:00:31.25	 & 0.0215 & 92 & 0.43 & FRI (LERG) &\citet{2001MNRAS.326.1499H}\\
  3C 83.1 & 0315+416 & 03:18:15.669	 & +41:51:27.91	 & 0.0251 & 108 & 0.50 & FRI (LERG)&\citet{2005ApJ...633..165S} \\
  3C 88 & 0325+023 & 03:27:54.194 & +02:33:41.98 & 0.0302 & 134 & 0.61 & FR I (NLRG) &\citet{2009ApJ...704.1586S}\\
  3C 120 & 0430+052 & 04:33:11.098	 & +05:21:15.59	 & 0.0330 & 143 & 0.65 & FR I (BLRG) &\citet{harris2004x}\\
  OJ 287 & 0851+202 & 08:54:48.875	 & +20:06:30.64	 & 0.3060 & 1576 & 4.48 & BL Lac &\citet{2011ApJ...729...26M}\\
  M84 & 1222+131 & 12:25:03.743 & +12:53:13.14 & 0.0034 & 17 & 0.08& FRI (LERG)&\citet{harris2002b} \\
  M87 & 1228+216 & 12:30:49.423	 & +12:23:28.04 & 0.0043 & 16 & 0.08 & FRI (NLRG) &\citet{Marshall_2002}\\
  3C 371 & 1807+698 & 18:06:50.590	 & +69:49:28.10	 & 0.0510 & 224 & 0.98 & BL Lac &\citet{pesce2001detection}\\
  S5 2007+777 & 2007+777 & 20:05:30.998 & +77:52:43.25 & 0.3420 & 1796 & 4.80 & BL Lac &\citet{2008ApJ...684..862S}\\
  PKS 2201+044 & 2201+044 & 22:04:17.651 & +04:40:02.05 & 0.0270 & 116 & 0.53 & BL Lac &\citet{2007ApJ...670...74S}\\
  3C465 & 2335+267 & 23:38:29.383 & +27:01:53.26 & 0.0293 & 126.6 & 0.57 & FRI (LERG)&\citet{hardcastle2005chandra}\\
  \enddata
  
 \tablecomments{All the cosmological parameters are taken from NASA/IPAC Extragalctic Database(NED)}
\tablenotetext{a}{Commonly used name for this source}
\tablenotetext{b}{IAU 1950 designation of the source}
\tablenotetext{c}{The celestial positions of the source in J2000 coordinates taken from NED}
\tablenotetext{d}{Redshift measurements taken from NED}
\tablenotetext{e}{The class column gives a radio jet morphology descriptor: Fanaroff-Riley I or II, CDQ (core dominated quasar), LDQ (Lobe dominated quasar), BL Lac, and an optical spectroscopic designation: LERG (low-excitation radio galaxy), HERG (high-excitation radio galaxy), NLRG (Narrow-line radio galaxy),BLRG (broad-line radio galaxy)  }
\tablenotetext{f}{The first publication in which a source shows a \textit{Chandra} detected X-ray component.}
%% General table references marker
%\tablerefs{\ref{test}}
\end{deluxetable*}
%\end{longrotatetable}


==> list_of_sources_copy.tex <==
\begin{tabular}{|l|l|l|l|r|r|r|l|}
\hline
  \multicolumn{1}{|c|}{Name} &
  \multicolumn{1}{c|}{IAU Name} &
  \multicolumn{1}{c|}{Ra} &
  \multicolumn{1}{c|}{Dec} &
  \multicolumn{1}{c|}{z} &
  \multicolumn{1}{c|}{\$D\_L\$} &
  \multicolumn{1}{c|}{Scale (kpc/arcsec)} &
  \multicolumn{1}{c|}{Type} \\
\hline
  3C6.1 & 0013+790 & 00:16:31 & +79:16:49.9 & 0.8404 & 5342.0 & 7.845 & FRII RG\\
  3C9 & 0017+154 & 00:20:25 & +15:40:54.7 & 2.012 & 15850.0 & 8.575 & LDQ\\
  3C13 & 0031+391 & 0:34:14.5560 & 39:24:16.6500 & 1.351 & 9830.0 & 8.633 & FR II\\
  3C15 & 0034-014 & 00:37:04 & -01:09:08.5 & 0.073 & 326.0 & 1.4 & FRI RG\\
  3C17 & 0035-024 & 00:38:21 & -02:07:40.7 & 0.22 & 1081.0 & 3.64 & FR2 RG\\
  3C29 & 0055+016 & 0:57:34.9160 & -1:23:27.9200 & 0.04503 & 201.0 & 0.893 & FR I\\
  NGC315 & 0055+300 & 00:57:49 & +30:21:08.8 & 0.0165 & 70.6 & 0.325 & FRI RG\\
  3C31 & 0104+321 & 01:07:25 & +32:25:45.0 & 0.0167 & 71.4 & 0.34 & FRI RG\\
  0106+013 & 0106+013 & 01:08:39 & +01:35:0.317 & 2.099 & 16702.0 & 8.43 & CDQ\\
  3C33 & 0106+130 & 01:08:53 & +13:20:13.8 & 0.0597 & 264.0 & 1.14 & FRII RG\\
  3C47 & 0133+207 & 01:36:24 & +20:57:27.4 & 0.425 & 2322.0 & 5.5 & LDQ\\
  3C66B & 0220+427 & 02:23:11 & +43:00:31.2 & 0.0215 & 92.0 & 0.43 & FRI RG\\
  0234+285 & 0234+285 & 02:37:52 & +28:48:08.9 & 1.213 & 8445.0 & 8.36 & CDQ\\
  3C83.1 & 0315+41 & 03:18:16 & +41:51:27.9 & 0.0251 & 108.0 & 0.5 & FRI RG\\
  3C88 & 0325+023 & 3:27:54.1948 & 2:33:41.9820 & 0.03022 & 134.0 & 0.614 & FR I\\
  PKS0405-12 & 0405-113 & 04:07:48 & -12:11:36.6 & 0.574 & 3338.0 & 6.5 & CDQ\\
  3C109 & 0410+11 & 04:13:40 & +11:12:13.8 & 0.3056 & 1574.0 & 4.5 & FRII RG\\
  3C111 & 0415+379 & 04:18:21 & +38:01:35.8 & 0.0491 & 215.0 & 0.95 & FRII RG\\
  3C120 & 0430+052 & 04:33:11 & +05:21:15.6 & 0.033 & 143.0 & 0.65 & Sy I\\
  3C123 & 0433+295 & 04:37:04 & +29:40:13.7 & 0.2177 & 1068.0 & 3.49 & FRII RG\\
  0454-463 & 0454-463 & 04:55:51 & -46:15:58.7 & 0.858 & 5481.0 & 7.7 & CDQ\\
  3C133 & 0459+252 & 5:2:58.4830 & 25:16:25.1100 & 0.2775 & 1460.0 & 4.346 & FR II\\
  PictorA & 0518-45 & 05:19:50 & -45:46:44.5 & 0.035 & 152.0 & 0.69 & FRII RG\\
  0529+075 & 0529+075 & 05:32:39 & +07:32:43.3 & 1.254 & 8803.0 & 8.4 & CDQ\\
  PKS0605-08 & 0605-08 & 06:08:00 & -08:34:49.9 & 0.87 & 5577.0 & 7.7 & CDQ\\
  PKS0637-752 & 0637-752 & 06:35:46 & -75:16:16.8 & 0.651 & 3909.0 & 6.9 & CDQ\\
  3C173.1 & 0702+749 & 07:09:18 & +74:49:31.8 & 0.292 & 1494.0 & 4.3 & FRII RG\\
  3C179 & 0723+679 & 07:28:12 & +67:48:47.5 & 0.846 & 5386.0 & 7.7 & LDQ\\
  B20738+313 & 0738+313 & 07:41:11 & +31:12:00.2 & 0.631 & 3777.0 & 6.9 & CDQ\\
  0827+243 & 0827+243 & 08:30:52 & +24:10:59.8 & 0.939 & 6133.0 & 7.9 & CDQ\\
  TXS0833+585 & 0833+585 & 8:37:22.4097 & 58:25:1.8450 & 2.101 & 16900.0 & 8.531 & Q\\
  4C+29.30 & 0836+2959 & 08:40:02 & +29:49:00.5 & 0.064 & 284.0 & 1.2 & FRI RG\\
  3C207 & 0837+133 & 08:40:47 & +13:12:23.0 & 0.68 & 4109.0 & 7.1 & LDQ\\
  OJ287 & 0851+20 & 08:54:49 & +20:06:30.6 & 0.306 & 1576.0 & 4.48 & BL Lac\\
  PKS0920-397 & 0920-397 & 09:08:17 & +39:43:26 & 1.88 & 14574.0 & 8.5 & FRII RG\\
  3C227 & 0945+07 & 09:47:45 & +07:25:20.6 & 0.0861 & 388.0 & 1.59 & FRII RG\\
  3C228 & 0947+145 & 9:50:10.7910 & 14:20:0.6300 & 0.5524 & 3300.0 & 6.62 & FR II\\
  4C +55.17 & 0954+556 & 9:57:38.1844 & 55:22:57.7690 & 0.89961 & 5960.0 & 8.009 & FR II\\
  Q0957+561 & 0957+561 & 10:01:21 & +55:53:56.5 & 1.41 & 10191.0 & 8.5 & LDQ\\
  4C+13.41 & 1004+130 & 10:07:26 & +12:48:56.2 & 0.24 & 1193.0 & 3.76 & LDQ\\
  PKS1030-357 & 1030-357 & 10:33:08 & -36:01:56.8 & 1.455 & 10599.0 & 8.53 & CDQ\\
  1045-188 & 1045-188 & 10:48:07 & -19:09:35.7 & 0.595 & 3487.0 & 6.64 & CDQ\\
  PKS1046-409 & 1046-409 & 10:48:38 & -41:13:59.6 & 0.62 & 3668.0 & 6.78 & CDQ\\
  PKS1055+201 & 1055+201 & 10:58:18 & +19:51:50.9 & 1.11 & 7558.0 & 8.2 & LDQ\\
  3C254 & 1111+408 & 11:14:38 & +40:37:20.3 & 0.734 & 4516.0 & 7.3 & LDQ\\
  PKS1127-145 & 1127-145 & 11:30:07 & -14:49:27.4 & 1.18 & 8159.0 & 8.3 & CDQ\\
  PKS1136-135 & 1136-135 & 11:39:11 & -13:50:43.6 & 0.554 & 3197.0 & 6.4 & LDQ\\
  3C263 & 1137+77 & 11:39:57 & +65:47:49.4 & 0.6563 & 3934.0 & 7.0 & LDQ\\
  3C265 & 1142+31 & 11:45:29 & +31:33:49.4 & 0.811 & 5110.0 & 7.55 & FRII RG\\
  4C+49.22 & 1150+497 & 11:53:24 & +49:31:06.9 & 0.334 & 1746.0 & 4.8 & CDQ\\
  3C268.1 & 1157+732 & 12:0:19.2100 & 73:0:45.7000 & 0.97 & 6540.0 & 8.17 & FR II\\
  PKS1202-262 & 1202-262 & 12:05:33 & -26:34:04.5 & 0.789 & 4939.0 & 7.48 & CDQ\\
  3C270.1 & 1218+339 & 12:20:33.8750 & 33:43:12.0500 & 1.52843 & 11500.0 & 8.69 & \\
  1222+216 & 1222+216 & 12:24:55 & +21:22:46.4 & 0.432 & 2367.0 & 5.6 & CDQ\\
  M84 & 1222+131 & 12:25:04 & +12:53:13.1 & 0.00339 & 17.0 & 0.082 & FRI RG\\
  3C273 & 1222+02 & 12:29:07 & +02:03:08.6 & 0.1583 & 749.0 & 2.7 & CDQ\\
  M87 & 1228+216 & 12:30:49 & +12:23:28.0 & 0.00427 & 16.0 & 0.077 & FRI RG\\
  PKS1229-02 & 1229-02 & 12:32:00 & -02:24:05.3 & 1.045 & 7009.0 & 8.1 & CDQ\\
  3C275.1 & 1241+26 & 12:43:58 & +16:22:53.2 & 0.555 & 3204.0 & 6.4 & LDQ\\
  3C277.3 & 1251+278 & 12:54:12.0130 & 27:37:33.9500 & 0.08534 & 406.0 & 1.668 & FR II\\
  PKS1311-270 & 1311-270 & 13:13:47.3570 & -27:16:49.2700 & 2.26 & 18500.0 & 8.436 & Q\\
  1317+520 & 1317+520 & 13:19:46 & +51:48:05.8 & 1.06 & 7135.0 & 8.15 & CDQ\\
  4C+11.45 & 1318+113 & 13:21:18.8380 & 11:6:49.9800 & 2.1792 & 17700.0 & 8.486 & Q\\
  CenA & 1322-428 & 13:25:28 & -43:01:08.8 & 0.001825 & 3.8 & 0.018 & FRI RG\\
  4C+65.15 & 1323+655 & 13:25:30 & +65:15:13.5 & 1.625 & 12163.0 & 8.6 & LDQ\\
  3C287.1 & 1330+022 & 13:32:53.2700 & 2:0:45.7000 & 0.215567 &  & 3.619 & FR II\\
  1334-127 & 1334-127 & 13:37:40 & -12:57:24.7 & 0.539 & 3091.0 & 6.33 & CDQ\\
  CenB & 1343-601 & 13:46:49 & -60:24:29.9 & 0.013 & 55.5 & 0.26 & FRI RG\\
  4C+19.44 & 1354+195 & 13:57:04 & +19:19:07.4 & 0.72 & 4410.0 & 7.2 & CDQ\\
  3C294 & 1404+344 & 14:06:44 & +34:11:25.1 & 1.786 & 13677.0 & 8.5 & FRII RG\\
  3C295 & 1409+524 & 14:11:21 & +52:12:09.0 & 0.45 & 2486.0 & 5.7 & FRII RG\\
  3C299 & 1419+419 & 14:21:5.5800 & 41:44:48.5000 & 0.367 & 2030.0 & 5.252 & FR II\\
  B3 1428+422 & 1428+422 & 14:30:23.7416 & 42:4:36.4910 & 4.715 & 44600.0 & 6.616 & \\
  3C303 & 1441+522 & 14:43:03 & +52:01:37.3 & 0.141 & 659.0 & 2.5 & RG\\
  TXS1508+572 & 1508+572 & 15:10:2.9223 & 57:2:43.3760 & 4.30872 & 40100.0 & 6.895 & Q\\
  1508+572 & 1508+572 & 15:10:03 & +57:02:44.0 & 4.3 & 39809.0 & 6.9 & CDQ\\
  PKS1510-08 & 1510-08 & 15:12:50 & -09:05:59.7 & 0.361 & 1913.0 & 5.0 & CDQ\\
  AP Lib & 1514-241 & 15:17:42 & -24:22:19.5 & 0.0486 & 213.0 & 0.939 & BL Lac\\
  3C321 & 1529+24 & 15:31:44 & +24:04:19.0 & 0.096 & 435.0 & 1.8 & FRII RG\\
  3C325 & 1549+628 & 15:49:58.4240 & 62:41:21.6600 & 1.135 & 7940.0 & 8.443 & FR II\\
  3C327 & 1600+021 & 16:02:27 & +01:57:56.2 & 0.1039 & 474.0 & 1.89 & FRII RG\\
  4C+00.58 & 1603+001 & 16:05:46 & +00:25:50.6 & 0.059 & 261.0 & 1.1 & LDQ\\
  3C330 & 1609+660 & 16:09:37 & +65:56:43.6 & 0.55 & 3169.0 & 6.4 & FRII RG\\
  3C334 & 1618+377 & 16:20:21.8190 & 17:36:24.0100 & 0.5551 & 3310.0 & 6.631 & FR II\\
  4C+15.55 & 1622+158 & 16:25:14.3730 & 15:45:21.9400 & 1.406 & 10300.0 & 8.659 & FR II\\
  NGC6251 & 1637+826 & 16:32:32 & +82:32:16.5 & 0.02488 & 107.0 & 0.49 & FRI/II RG\\
  1642+690 & 1642+690 & 16:42:08 & +68:56:39.7 & 0.751 & 4646.0 & 7.3 & CDQ\\
  3C345 & 1641+399 & 16:42:59 & +39:48:37.0 & 0.594 & 3481.0 & 6.6 & CDQ\\
  3C346 & 1641+173 & 16:43:49 & +17:15:49.0 & 0.161 & 762.6 & 2.74 & FRI RG\\
  3C351 & 1704+605 & 17:04:41 & +60:44:30.7 & 0.372 & 1982.0 & 5.1 & LDQ\\
  1745+624 & 1745+624 & 17:46:14 & +62:26:54.7 & 3.889 & 35316.0 & 7.2 & LDQ\\
  1800+440 & 1800+440 & 18:01:32 & +44:04:21.9 & 0.663 & 3983.0 & 6.98 & CDQ\\
  3C371 & 1807+698 & 18:06:51 & +69:49:28.1 & 0.051 & 224.0 & 0.98 & BL Lac\\
  3C390.3 & 1845+797 & 18:42:09 & +79:46:17.2 & 0.0561 & 247.0 & 1.08 & FRII RG\\
  1849+670 & 1849+670 & 18:49:16 & +67:05:41.7 & 0.657 & 3938.0 & 6.95 & CDQ\\
  1928+738 & 1928+738 & 19:27:48 & +73:58:01.6 & 0.302 & 1553.0 & 4.4 & CDQ\\
  3C403 & 1949+023 & 19:52:16 & +02:30:24.4 & 0.059 & 260.6 & 1.127 & FRII RG\\
  CygA & 1957+405 & 19:59:28 & +40:44:01.9 & 0.056 & 247.0 & 1.07 & FRII RG\\
  S52007+777 & 2007+777 & 20:05:31 & +77:52:43 & 0.342 & 1796.0 & 4.8 & BL Lac\\
  4C+74.26 & 2043+749 & 20:42:37 & +75:08:02.5 & 0.104 & 474.0 & 1.9 & LDQ\\
  2155-152 & 2155-152 & 21:58:06 & -15:01:09.3 & 0.672 & 4049.0 & 7.02 & CDQ\\
  PKS2201+044 & 2201+044 & 22:04:18 & +04:40:02.0 & 0.027 & 116.0 & 0.535 & BL Lac\\
  2209+080 & 2209+080 & 22:12:02 & +08:19:16.5 & 0.485 & 2721.0 & 5.98 & CDQ\\
  2216-038 & 2216-038 & 22:18:52 & -03:35:36.9 & 0.901 & 5825.0 & 7.81 & CDQ\\
  3C445 & 2221-02 & 22:23:50 & -02:06:12.4 & 0.056 & 247.0 & 1.1 & FRII RG\\
  3C452 & 2243+394 & 22:45:49 & +39:41:15.7 & 0.0811 & 364.0 & 1.5 & FRII RG\\
  3C454.3 & 2252+15 & 22:53:58 & +16:08:53.6 & 0.859 & 5489.0 & 7.7 & CDQ\\
  3C465 & 2335+46 & 23:38:29 & +27:01:55.9 & 0.0293 & 126.6 & 0.579 & FRI RG\\
\hline\end{tabular}


==> offsets_table.tex <==
%\textcolor{blue}{Add the proper references}
\startlongtable
\tablecolumns{11}
\centerwidetable 
\begin{deluxetable*}{ll|LlC|LLCCCC}
  %\centerwidetable
  \tabletypesize{\scriptsize}
  \tablecaption{Results from offset the analysis and spectral data\label{table:offset-results}}
  \tablehead{
    \colhead{Name} &
    \colhead{Component}&
    %\nocolhead{Common name\textsuperscript{b}} &
    \multicolumn{3}{c}{Offset} &
    \colhead{$\alpha_r$}&
    \colhead{$\alpha_X$}&
    \colhead{$\nu_r$} &
    \colhead{$f_r$} &
    \colhead{$f_{1 keV}$}&
    \colhead{$R$}\\[-5pt]
    \colhead{}&
    \colhead{}&
    \colhead{$\arcsec$}&
    \colhead{Type\textsuperscript{b}}&
    \colhead{kpc\textsuperscript{c}}&
    \colhead{}&
    \colhead{}&
    \colhead{GHz}&
    \colhead{mJy}&
    \colhead{nJy}&
    \colhead{$\log_{10}(\frac{\nu_XF_X}{\nu_rF_r})$}\\
  }
    \startdata
    3C 9 & H & 0.29\pm0.09  & Xf+Bnd & 2.46\pm0.77 &  &  & 14.99 & 47.20 & 0.30  & 0.10 \\
    3C15 & B & 0.66\pm0.29  & Xf+Flr & 0.92\pm0.40 &  &  & 8.40 & 33.20 & 0.64  & 0.56 \\
     & C & 0.14\pm0.04  & Co-s & 0.20\pm0.06 & 0.90 & 0.70\pm0.36 ~(32) & 8.40 & 8.30 & 1.10  & 3.82 \\
    3C 31 & B & 0.77\pm0.05  & Xf+Flr & 0.26\pm0.02 & 0.55 & 1.30\pm0.20  & 8.46 & 6.83 & 2.45  & 10.25 \\
    4C +01.02 & B & 0.12\pm0.07  & Co-s+Bnd & 0.97\pm0.56 & 1.02 & 0.80\pm0.30 ~(1) & 4.80 & 10.04 & 4.55 ~(1) & 22.85 \\
     & SHS & 0.40\pm0.06 ~(1) & Xf & 3.41\pm0.50 & 1.02 & 0.90\pm0.60 ~(1) & 4.80 & 114.60 & 1.72 ~(1) & 0.76 \\
    3C 47 & SHS & 0.20\pm0.13  & Co-s+Bnd & 1.07\pm0.72 &  &  & 4.84 & 212.00 & 0.54 ~(3) & 0.13 \\
    PKS 0144-522 & A & 0.19\pm0.15  & Co-s & 0.35\pm0.28 &  &  & 17.73 & 2.78 & 1.02  & 4.98 \\
    4C +35.03 & A & 0.47\pm0.18  & Rf & 0.34\pm0.13 &  &  & 4.86 & 16.96 & 1.56  & 4.58 \\
    PKS 0208-512 & K3 & 0.13\pm0.30  & Co-s & 1.05\pm2.41 & 0.50 & 0.62\pm0.12  & 8.64 & 59.60 & 4.07 ~(4) & 1.91 \\
    3C 66B & B & 0.42\pm0.06 ~(5) & Xf+Flr & 0.18\pm0.03 & 0.60 &  & 8.21 & 17.70 & 6.10 ~(5) & 10.16 \\
     & C & 0.29\pm0.10  & Xf & 0.12\pm0.04 &  &  & 8.21 & 6.78 & 0.74  & 3.23 \\
     & D & 0.14\pm0.05  & Co-s & 0.06\pm0.02 &  &  & 8.21 & 1.18 & 1.45  & 36.17 \\
     & A & \cdots & (T)Co-s & \cdots & 0.75 & 0.97\pm0.34 ~(5) & 8.21 & 1.60 & 4.00 ~(5) & 73.69 \\
    4C +28.07 & D & \cdots & (T)Co-s & \cdots &  &  & 8.47 & 5.86 & 1.92  & 9.37 \\
     & C & \cdots & (T)Co-s & \cdots &  &  & 8.47 & 6.42 & 6.64  & 29.53 \\
     & NHS-a & 1.17\pm0.12  & Xf+Jet-HS & 9.76\pm1.01 &  &  & 8.47 & 35.70 & 1.06  & 0.85 \\
    3C 78 & C & 0.10\pm0.01  & Co-s & 0.06\pm0.01 &  &  & 8.46 & 72.80 & 17.83  & 7.00 \\
    3C 83.1 & E1 & 0.72\pm0.12  & Xf & 0.36\pm0.06 &  & 0.71\pm0.40  & 4.98 & 13.77 & 0.19  & 0.68 \\
     & W1 & 0.65\pm0.22  & Xf & 0.33\pm0.11 &  & 1.13\pm0.53  & 4.98 & 3.55 & 0.19  & 2.55 \\
    3C 88 & C & 1.14\pm0.23  & Xf & 0.70\pm0.14 &  &  & 4.83 & 47.70 & 0.36  & 0.38 \\
    PKS 0405-12 & NHS & 0.12\pm0.08  & Co-s & 0.78\pm0.51 & 0.90\pm 0.10 &  & 8.46 & 115.00 & 1.90  & 0.47 \\
    PKS 0413-21 & A & 0.24\pm0.08  & Xf & 1.81\pm0.60 &  &  & 8.46 & 258.00 & 5.35  & 0.59 \\
    3C 111 & NHS & 0.56\pm0.10 ~(6) & Xf & 0.53\pm0.10 &  & 0.83\pm0.28 ~(6) & 8.40 & 610.31 & 3.72 ~(6) & 0.18 \\
     & K97 & 0.52\pm0.10  & Amb & 0.49\pm0.10 &  &  & 8.40 & 27.88 & 1.18 ~(6) & 1.22 \\
     & K61 & 0.91\pm0.16 ~(6) & Xf & 0.86\pm0.15 &  & 1.01\pm0.21 ~(6) & 8.40 & 38.13 & 8.76 ~(6) & 6.62 \\
     & K45 & 0.47\pm0.69  & Co-s & 0.45\pm0.66 &  &  & 8.40 & 11.96 & 1.10 ~(6) & 2.65 \\
     & K30 & 0.87\pm0.09 ~(6) & Xf & 0.83\pm0.09 &  & 0.79\pm0.30 ~(6) & 8.40 & 13.15 & 4.46 ~(6) & 9.77 \\
     & K14 & 2.00\pm0.25 ~(6) & Xf & 1.90\pm0.24 &  &  & 8.40 & 9.35 & 1.82 ~(6) & 5.61 \\
     & K9 & 0.27\pm0.13 ~(6) & Xf & 0.26\pm0.12 &  &  & 8.40 & 6.91 & 2.14 ~(6) & 8.92 \\
    3C 120 & K4 & 0.32\pm0.11  & Xf & 0.21\pm0.07 & 0.74\pm 0.04 & 0.90\pm0.20 ~(7) & 10.00 & 57.60 & 10.00 ~(7) & 4.20 \\
     & K7 & 0.17\pm0.22  & Co-s+Bnd & 0.11\pm0.14 & 0.68\pm 0.04 & 2.40\pm0.60 ~(7) & 10.00 & 12.98 & 6.30 ~(7) & 11.75 \\
    3C 123 & SHS & 0.37\pm0.06  & Xf+Jet-HS & 1.29\pm0.22 & 0.50 & 0.60\pm0.30 ~(8) & 8.44 & 2189.00 & 4.60 ~(8) & 0.06 \\
    PKS 0454-46 & A & 0.14\pm0.05  & Co-s+Bnd & 1.04\pm0.42 &  & 0.71\pm0.23  & 8.64 & 68.70 & 11.39  & 4.65 \\
    PKS 0605-089 & WHS & 1.02\pm0.06 ~(38) & Xf+Bnd & 7.85\pm0.46 &  & 0.43\pm0.11  & 9.99 & 18.50 & 11.62  & 15.21 \\
    PKS 0637-752 & D & 0.14\pm0.12  & Co-s & 0.97\pm0.83 &  &  & 17.73 & 20.30 & 1.26  & 0.85 \\
     & E & 0.17\pm0.15  & Co-s & 1.17\pm1.03 &  &  & 17.73 & 16.60 & 1.23  & 1.01 \\
     & F & 0.11\pm0.06  & Co-s & 0.76\pm0.41 &  &  & 17.73 & 33.30 & 6.30  & 2.58 \\
     & H & 0.09\pm0.11  & Co-s & 0.62\pm0.76 &  &  & 17.73 & 47.00 & 2.14  & 0.62 \\
     & G & 0.10\pm0.12  & Co-s & 0.69\pm0.83 &  &  & 17.73 & 47.00 & 8.57  & 2.49 \\
    B2 0738+313 & A & 0.54\pm0.13  & Xf & 3.72\pm0.91 &  & 0.54\pm0.37 ~(33) & 4.86 & 0.41 & 0.48  & 58.90 \\
    OJ 248 & C4 & 0.29\pm0.07 ~(39) & Xf & 2.31\pm0.57 & 1.13\pm 0.10 &  & 4.86 & 0.26 & 0.97  & 185.60 \\
     & C2 & 0.08\pm0.05  & Co-s+Bnd & 0.63\pm0.36 &  &  & 4.86 & 0.18 & 1.89  & 515.30 \\
    4C +29.30 & NHS-a & 0.09\pm0.05  & Co-s & 0.11\pm0.06 & 0.85\pm 0.10 & 2.34\pm0.16 ~(34) & 4.80 & 8.78 & 1.05  & 6.01 \\
     & A & 0.32\pm0.11 ~(34) & Xf & 0.38\pm0.13 &  &  & 4.80 & 5.36 & 0.23  & 2.15 \\
     & SHS & 0.12\pm0.02  & Co-s & 0.14\pm0.03 &  & 1.16\pm0.08 ~(34) & 4.80 & 12.65 & 2.13  & 8.47 \\
    3C 207 & F & 0.35\pm0.06  & Rf+Bnd & 2.48\pm0.43 & 0.80 & 0.23\pm0.33  & 14.99 & 55.70 & 4.60  & 1.33 \\
     & WHS & 0.33\pm0.09  & Xf & 2.32\pm0.62 & 0.80 & 0.64\pm0.38  & 14.99 & 16.80 & 1.30  & 1.25 \\
    OJ 287 & J1 & 0.51\pm0.23  & Rf & 2.28\pm1.05 &  &  & 1.43 & 1.26 & 1.23  & 164.85 \\
     & J2 & 0.23\pm0.05 ~(40) & Rf & 1.04\pm0.24 &  & 0.65\pm0.09  & 1.43 & 3.08 & 6.36  & 349.61 \\
     & J4 & 0.47\pm0.06  & Xf & 2.11\pm0.26 &  & 0.69\pm0.11  & 1.43 & 1.71 & 6.03  & 596.75 \\
     & J3 & 0.36\pm0.09  & Xf+Bnd & 1.63\pm0.40 &  & 0.66\pm0.14  & 1.43 & 1.63 & 3.24  & 336.07 \\
    PKS 0920-397 & E & 0.23\pm0.13  & Co-s+Vnsh & 1.99\pm1.14 &  &  & 8.46 & 12.00 & 1.78  & 4.25 \\
     & C & \cdots & (T)Co-s & \cdots &  &  & 8.46 & 11.70 & 1.75  & 4.28 \\
     & SHS & 0.81\pm0.10  & Xf+Jet-HS & 6.88\pm0.89 &  & 0.87\pm0.52  & 8.46 & 15.20 & 1.81  & 3.40 \\
    3C 228 & SHS & 0.31\pm0.04  & Xf & 2.04\pm0.23 &  &  & 8.47 & 135.50 & 1.30 ~(3) & 0.27 \\
    Q 0957+561 & WHS & 0.74\pm0.18  & Xf & 6.27\pm1.57 &  &  & 8.44 & 40.80 & 0.16  & 0.11 \\
    PKS 1030-357 & E & 0.40\pm0.07  & Rf+Bnd & 3.37\pm0.62 &  & 1.27\pm0.21  & 18.94 & 6.29 & 3.88  & 7.87 \\
     & D & 0.27\pm0.07  & Xf+Bnd & 2.28\pm0.61 &  & 0.89\pm0.21  & 18.94 & 3.92 & 2.84  & 9.25 \\
     & C & 0.41\pm0.14  & Rf+Vnsh & 3.52\pm1.17 &  &  & 18.94 & 2.13 & 0.57  & 3.40 \\
     & B & 0.26\pm0.17  & Co-s & 2.22\pm1.45 &  &  & 18.94 & 3.66 & 0.36  & 1.26 \\
     & F & 0.31\pm0.11  & Xf+Bnd & 2.62\pm0.95 &  & 0.85\pm0.35  & 18.94 & 5.37 & 0.96  & 2.29 \\
    PKS 1045-188 & H & 0.20\pm0.04  & Xf+Bnd & 1.36\pm0.27 &  & 0.81\pm0.30 ~(11) & 8.41 & 16.40 & 0.90 ~(11) & 1.58 \\
    PKS 1055+201 & A & 0.09\pm0.04  & Co-s & 0.70\pm0.34 &  & 0.83\pm0.14  & 4.98 & 15.00 & 1.08  & 3.51 \\
     & NHS-a & 0.11\pm0.04  & Co-s & 0.88\pm0.29 &  & 1.20\pm0.13  & 4.98 & 488.00 & 1.38  & 0.14 \\
     & NHS-b & 0.23\pm0.09  & Co-s & 1.84\pm0.72 &  &  & 4.98 & 370.00 & 0.19  & 0.02 \\
    3C 254 & EHS & 0.34\pm0.13  & Xf & 2.45\pm0.93 &  & 1.47\pm0.69  & 4.86 & 274.00 & 1.09  & 0.20 \\
    PKS 1127-145 & C & 0.50\pm0.26 ~(41) & Xf & 4.17\pm2.12 & 0.85\pm 0.08 & 0.83\pm0.41  & 8.46 & 12.20 & 0.33  & 0.76 \\
     & B & 0.47\pm0.13 ~(41) & Xf & 3.93\pm1.11 & 0.91\pm 0.07 & 0.89\pm0.20  & 8.46 & 6.01 & 0.84  & 3.98 \\
    PKS 1136-135 & A & 0.28\pm0.07 ~(12) & Xf & 1.80\pm0.45 & 0.67\pm 0.11 &  & 4.86 & 3.84 & 1.70 ~(12) & 22.04 \\
     & EHS & 0.35\pm0.17  & Xf+Jet-HS & 2.23\pm1.06 & 0.85\pm 0.08 &  & 4.86 & 207.00 & 0.32 ~(12) & 0.08 \\
     & B & \cdots & (T)Co-s & \cdots & 0.81\pm 0.13 &  & 4.86 & 10.90 & 3.50 ~(12) & 15.99 \\
     & E & \cdots & (T)Co-s & \cdots & 0.82\pm 0.09 &  & 4.86 & 111.50 & 0.70 ~(12) & 0.31 \\
     & alpha & 0.37\pm0.10  & Xf & 2.39\pm0.61 & 0.75\pm 0.10 &  & 4.86 & 2.56 & 1.90 ~(12) & 36.96 \\
     & C & \cdots & (T)Co-s & \cdots & 0.66\pm 0.09 &  & 4.86 & 31.50 & 1.80 ~(12) & 2.85 \\
    3C 263 & WHS & 0.28\pm0.07  & Xf & 1.94\pm0.46 & 0.84 & 1.07\pm0.21 ~(13) & 4.86 & 534.60 & 1.70 ~(13) & 0.16 \\
    3C 265 & E & 0.19\pm0.11  & Co-s & 1.43\pm0.82 & 1.17\pm 0.11 & 1.06\pm0.49  & 8.44 & 166.40 & 0.36  & 0.06 \\
    4C +49.22 & H & 0.12\pm0.03  & Co-s & 0.56\pm0.13 & 0.72\pm 0.09 & 0.64\pm0.20  & 4.86 & 9.74 & 1.00 ~(12) & 5.11 \\
     & E & 0.10\pm0.01  & Co-s & 0.46\pm0.06 & 0.67\pm 0.08 & 0.69\pm0.17  & 4.86 & 3.37 & 1.70 ~(12) & 25.12 \\
     & D & 0.12\pm0.04  & Co-s & 0.55\pm0.20 & 0.68\pm 0.10 & 0.86\pm0.19  & 4.86 & 4.22 & 1.30 ~(12) & 15.34 \\
     & B & 0.20\pm0.03  & Xf & 0.95\pm0.12 & 0.72\pm 0.09 & 0.73\pm0.20 ~(12) & 4.86 & 6.48 & 7.60 ~(12) & 58.40 \\
    PKS 1202-262 & B & \cdots & (T)Co-s & \cdots &  &  & 4.86 & 13.30 & 1.73  & 6.49 \\
     & D & \cdots & (T)Co-s & \cdots &  &  & 4.86 & 11.40 & 2.31  & 10.10 \\
     & C & \cdots & (T)Co-s & \cdots &  &  & 4.86 & 9.93 & 1.27  & 6.35 \\
     & NHS & 0.28\pm0.02 ~(42) & Xf+Jet-HS & 2.11\pm0.16 &  &  & 4.86 & 40.10 & 10.70  & 13.29 \\
    3C 270.1 & SHS & 0.38\pm0.05 ~(14) & Xf+Jet-HS & 3.26\pm0.40 &  & 0.66\pm0.16  & 8.40 & 158.00 & 1.41 ~(14) & 0.26 \\
     & NHS-a & 0.26\pm0.12  & Co-s+Jet-HS & 2.24\pm1.03 &  &  & 8.40 & 7.26 & 0.33 ~(14) & 1.31 \\
    M84 & B & 1.37\pm0.10  & Xf & 0.11\pm0.01 & 0.65 &  & 8.40 & 9.50 & 0.66 ~(15) & 2.00 \\
     & A & 0.60\pm0.11  & Xf+Flr & 0.05\pm0.01 & 0.65 &  & 8.40 & 1.84 & 0.60 ~(15) & 9.39 \\
    4C +21.35 & C2 & 0.19\pm0.03  & Xf+Bnd & 1.07\pm0.17 &  &  & 8.46 & 29.60 & 11.61  & 11.22 \\
    M87 & B & 0.19\pm0.05 ~(17) & Xf & 0.01\pm0.00 &  & 1.28\pm0.24 ~(35) & 9.99 & 1440.00 & 19.20 ~(17) & 0.32 \\
     & A & 0.03\pm0.03  & Co-s & 0.00\pm0.00 &  & 1.32\pm0.01 ~(35) & 9.99 & 1720.00 & 142.00 ~(17) & 2.00 \\
     & I & 0.23\pm0.03 ~(17) & Xf & 0.02\pm0.00 &  &  & 9.99 & 270.00 & 6.48  & 0.58 \\
     & E & 0.18\pm0.10  & Co-s & 0.01\pm0.01 &  & 1.32\pm0.26 ~(35) & 9.99 & 200.00 & 15.40 ~(17) & 1.87 \\
     & D & 0.21\pm0.01 ~(17) & Xf & 0.02\pm0.00 &  & 1.04\pm0.16 ~(35) & 9.99 & 230.00 & 67.90 ~(17) & 7.15 \\
     & F & 0.40\pm0.05 ~(17) & Xf & 0.03\pm0.00 &  & 1.90\pm0.44 ~(35) & 9.99 & 300.00 & 10.00 ~(17) & 0.81 \\
     & C & 0.36\pm0.02 ~(17) & Xf & 0.03\pm0.00 &  & 1.54\pm0.88 ~(35) & 9.99 & 1550.00 & 7.20 ~(17) & 0.11 \\
    PKS 1229-02 & C & 0.16\pm0.01  & Xf+Bnd & 1.28\pm0.05 &  &  & 8.52 & 37.40 & 2.79  & 2.12 \\
     & EHS & 0.53\pm0.14  & Xf & 4.32\pm1.11 &  &  & 8.52 & 29.20 & 0.57  & 0.56 \\
    3C 275.1 & EHS & 0.41\pm0.06  & Xf & 2.64\pm0.38 & 0.69\pm 0.12 & 0.86\pm0.21  & 4.86 & 193.80 & 1.78 ~(3) & 0.46 \\
    3C 277.3 & K2 & 0.27\pm0.03 ~(18) & Xf+Bnd & 0.45\pm0.05 & 0.67\pm 0.04 & 1.00\pm0.60 ~(18) & 4.87 & 12.60 & 0.40 ~(18) & 1.58 \\
     & NHS & 3.07\pm0.11 ~(18) & Xf+Jet-HS & 5.12\pm0.18 &  & 1.30\pm0.80 ~(18) & 4.87 & 98.50 & 0.70 ~(18) & 0.35 \\
    4C +52.27 & WHS & 0.26\pm0.06  & Xf & 2.09\pm0.46 &  & 0.88\pm0.05 ~(36) & 4.86 & 61.30 & 2.93  & 2.38 \\
    3C 287.1 & EHS & 2.39\pm0.21  & Xf+Jet-HS & 8.65\pm0.76 &  &  & 4.86 & 71.20 & 1.17  & 0.82 \\
     & A & 0.92\pm0.24  & Xf & 3.34\pm0.89 &  &  & 4.86 & 2.90 & 1.03  & 17.64 \\
    PKS 1335-127 & A & 0.12\pm0.08  & Co-s & 0.73\pm0.51 &  &  & 4.86 & 21.50 & 5.93  & 13.72 \\
     & B & 0.22\pm0.05  & Xf+Bnd & 1.41\pm0.34 &  & 0.63\pm0.15  & 4.86 & 28.40 & 13.56  & 23.77 \\
    4C +19.44 & S12.9 & 0.14\pm0.07  & Co-s & 1.00\pm0.53 & 0.78\pm 0.09 & 0.93\pm0.16 ~(19) & 4.86 & 9.91 & 0.64 ~(19) & 3.23 \\
     & S17.7 & 0.44\pm0.10 ~(19) & Rf+Vnsh & 3.20\pm0.68 & 0.93\pm 0.47 & 0.81\pm0.13 ~(19) & 4.86 & 2.48 & 0.86 ~(19) & 17.37 \\
     & S11.2 & 0.18\pm0.03  & Co-s & 1.27\pm0.24 & 0.87\pm 0.15 & 0.68\pm0.21 ~(19) & 4.86 & 5.34 & 0.31 ~(19) & 2.89 \\
     & S10 & \cdots & (T)Co-s & \cdots & 0.88\pm 0.14 & 0.61\pm0.20 ~(19) & 4.86 & 6.19 & 0.30 ~(19) & 2.43 \\
     & S8.3 & \cdots & (T)Co-s & \cdots & 0.83\pm 0.05 & 0.64\pm0.14 ~(19) & 4.86 & 19.00 & 0.69 ~(19) & 1.82 \\
     & S5.4 & \cdots & (T)Co-s & \cdots & 0.74\pm 0.09 & 0.90\pm0.22 ~(19) & 4.86 & 6.69 & 0.18 ~(19) & 1.37 \\
     & S4 & 0.12\pm0.07  & Co-s & 0.84\pm0.53 & 0.74\pm 0.05 & 0.55\pm0.13 ~(19) & 4.86 & 16.50 & 0.51 ~(19) & 1.55 \\
     & S14.6 & 0.24\pm0.14  & Co-s & 1.70\pm0.98 & 0.86\pm 0.09 & 0.88\pm0.17 ~(19) & 4.86 & 9.18 & 0.60 ~(19) & 3.28 \\
     & S25.7 & \cdots & (T)Co-s & \cdots &  &  & 4.86 & 2.64 & 0.09 ~(19) & 1.77 \\
     & SHS-a & \cdots & (T)Co-s & \cdots &  &  & 4.86 & 6.58 & 0.29 ~(19) & 2.22 \\
     & S15.9 & \cdots & (T)Co-s & \cdots & 0.83\pm 0.27 & 0.81\pm0.16 ~(19) & 4.86 & 2.79 & 0.58 ~(19) & 10.37 \\
     & SHS-b & 0.28\pm0.09 ~(19) & Xf & 1.98\pm0.67 &  &  & 4.86 & 85.70 & 1.09 ~(19) & 0.63 \\
    3C 294 & SHS & 0.49\pm0.17  & Xf+Jet-HS & 4.21\pm1.40 &  &  & 4.76 & 34.30 & 0.94 ~(3) & 1.39 \\
     & NHS & 0.40\pm0.18  & Xf+Jet-HS & 3.43\pm1.50 &  &  & 4.76 & 153.60 & 1.40 ~(3) & 0.46 \\
    3C 295 & SHS & 0.18\pm0.12  & Co-s & 1.05\pm0.66 &  &  & 8.56 & 1092.00 & 2.17  & 0.06 \\
     & NHS & 0.27\pm0.06  & Xf & 1.52\pm0.35 & 0.94\pm 0.10 &  & 8.56 & 995.00 & 5.21  & 0.15 \\
    3C 299 & EHS & 0.35\pm0.10  & Xf & 1.84\pm0.50 &  &  & 4.86 & 844.00 & 0.60  & 0.04 \\
    PKS B1421-490 & A1 & 0.10\pm0.02  & Co-s & 0.70\pm0.17 &  & 0.30\pm0.30 ~(20) & 20.16 & 1960.00 & 13.30 ~(20) & 0.08 \\
    3C 303 & HS-a & 0.14\pm0.08  & Co-s & 0.36\pm0.20 & 0.84\pm 0.10 & 0.40\pm0.20 ~(37) & 8.44 & 83.40 & 3.09  & 1.06 \\
     & C & 0.46\pm0.11  & Xf & 1.14\pm0.28 &  &  & 8.44 & 1.70 & 1.07  & 18.06 \\
     & B & 0.33\pm0.13  & Xf & 0.82\pm0.32 &  &  & 8.44 & 2.45 & 0.83  & 9.74 \\
     & A & 0.46\pm0.16  & Xf & 1.16\pm0.41 &  &  & 8.44 & 1.97 & 0.31  & 4.50 \\
    PKS 1510-08 & B & 0.06\pm0.04  & Co-s & 0.32\pm0.20 &  & 0.68\pm0.12  & 4.86 & 8.85 & 6.16  & 34.65 \\
    3C 325 & WHS & 0.12\pm0.07  & Co-s & 1.05\pm0.61 &  &  & 4.86 & 235.10 & 0.35  & 0.07 \\
     & EHS & 0.12\pm0.09  & Co-s & 1.00\pm0.75 &  &  & 4.86 & 264.00 & 0.36  & 0.07 \\
    4C +00.58 & C & 0.21\pm0.03  & Xf+Bnd & 0.23\pm0.04 &  & 0.60\pm0.40  & 9.99 & 5.73 & 0.40  & 1.70 \\
     & D & 0.05\pm0.02  & Co-s+Bnd & 0.06\pm0.02 &  & 1.10\pm0.22  & 9.99 & 6.92 & 0.94  & 3.29 \\
    3C 330 & NHS & 0.27\pm0.10  & Xf & 1.75\pm0.61 &  &  & 4.85 & 818.00 & 0.34 ~(13) & 0.02 \\
    4C +15.55 & SHS & 0.29\pm0.11  & Xf & 2.52\pm0.92 &  &  & 4.80 & 120.30 & 0.29  & 0.12 \\
     & C & 0.17\pm0.08  & Co-s+Bnd & 1.43\pm0.70 &  &  & 4.80 & 43.20 & 0.53  & 0.62 \\
    3C 346 & B & 0.22\pm0.03 ~(21) & Xf & 0.60\pm0.08 &  & 1.00\pm0.30 ~(21) & 4.86 & 184.30 & 1.60 ~(21) & 0.43 \\
    3C 345 & NHS & 0.17\pm0.03 ~(1) & Xf & 1.09\pm0.17 &  & 0.89\pm0.18  & 8.44 & 114.80 & 3.18  & 0.80 \\
     & D & 0.10\pm0.09  & Co-s & 0.63\pm0.60 & 0.55 &  & 8.44 & 53.40 & 0.70  & 0.37 \\
    4C +69.21 & D & 0.22\pm0.12  & Co-s & 1.61\pm0.89 &  &  & 8.44 & 19.07 & 0.46  & 0.69 \\
     & C & 0.07\pm0.04  & Co-s & 0.53\pm0.33 &  &  & 8.44 & 23.64 & 2.71  & 3.29 \\
    3C 351  & L & 0.33\pm0.04 ~(22) & Amb & 1.67\pm0.23 & 0.70 & 1.00\pm0.13  & 8.44 & 303.00 & 3.40 ~(22) & 0.32 \\
     & J & 0.34\pm0.02 ~(22) & Amb & 1.71\pm0.10 & 0.75 & 0.86\pm0.11  & 8.44 & 134.60 & 5.20 ~(22) & 1.11 \\
    1800+440 & EHS & 0.02\pm0.09  & Co-s & 0.12\pm0.64 &  & 0.92\pm0.23  & 8.44 & 33.90 & 6.42  & 5.43 \\
    4C +56.27 & B & 0.14\pm0.08  & Co-s & 1.01\pm0.59 &  &  & 4.86 & 82.00 & 6.70  & 4.07 \\
    3C 380 & HS & \cdots & (T)Co-s & \cdots &  &  & 4.86 & 1426.00 & 51.70  & 1.81 \\
    1849+670 & A & 0.39\pm0.22  & Amb & 2.71\pm1.55 &  &  & 9.99 & 0.81 & 0.41  & 12.16 \\
     & C & 0.16\pm0.10  & Co-s & 1.13\pm0.67 &  &  & 9.99 & 0.46 & 0.69  & 35.90 \\
    4C +73.18 & A & 0.24\pm0.05  & Xf+Bnd & 1.06\pm0.23 &  & 0.89\pm0.15  & 4.86 & 6.98 & 7.18  & 51.25 \\
    3C 403 & F1 & 0.30\pm0.13 ~(24) & Xf & 0.34\pm0.15 &  &  & 8.35 & 34.50 & 0.90 ~(24) & 0.76 \\
     & F6 & 0.48\pm0.10 ~(24) & Xf & 0.54\pm0.11 &  &  & 8.35 & 41.60 & 2.30 ~(24) & 1.60 \\
    S5 2007+777 & K15.9 & 0.77\pm0.24  & Xf & 3.71\pm1.17 &  & 0.22\pm0.32  & 1.43 & 3.98 & 0.44 ~(26) & 18.71 \\
     & K11.1 & 0.53\pm0.17  & Rf & 2.54\pm0.83 &  & 0.11\pm0.37  & 1.43 & 3.90 & 0.38 ~(26) & 16.49 \\
     & K8.5 & 0.14\pm0.09  & Co-s & 0.66\pm0.45 &  &  & 1.43 & 4.55 & 0.90 ~(26) & 33.47 \\
    PKS 2101-490 & K3 & 0.07\pm0.10  & Co-s & 0.57\pm0.81 &  &  & 17.73 & 3.50 & 0.50 ~(28) & 1.95 \\
     & HS & 0.83\pm0.17 ~(28) & Xf & 6.76\pm1.38 &  &  & 17.73 & 16.00 & 0.75 ~(28) & 0.64 \\
    PKS 2152-69 & NHS & 1.01\pm0.12 ~(45) & Xf & 0.57\pm0.07 &  & 0.80\pm0.30 ~(29) & 18.00 & 33.40 & 1.00 ~(29) & 0.40 \\
     & D & 0.17\pm0.01 ~(45) & Xf & 0.10\pm0.01 &  & 1.20\pm0.40 ~(29) & 18.00 & 8.20 & 1.30 ~(29) & 2.13 \\
    4C +08.64 & E & 0.48\pm0.10  & Xf+Bnd & 2.89\pm0.60 & 0.71 & 1.19\pm0.32  & 4.80 & 40.70 & 1.92  & 2.38 \\
    4C -03.79 & C & 0.15\pm0.09  & Co-s+Bnd & 1.19\pm0.72 &  & 0.17\pm0.36  & 6.00 & 26.90 & 0.50  & 0.75 \\
     & B & 0.37\pm0.16  & Rf & 2.92\pm1.23 &  & 0.44\pm0.26  & 6.00 & 9.01 & 1.30  & 5.82 \\
    3C 452 & EHS & 1.37\pm0.24 ~(3) & Xf & 2.06\pm0.36 &  & 0.93\pm0.30  & 8.40 & 61.70 & 0.34 ~(3) & 0.16 \\
    3C 454.3 & NHS & 0.26\pm0.01  & Xf+Jet-HS & 2.03\pm0.11 &  & 0.67\pm0.14  & 8.40 & 130.00 & 6.00 ~(31) & 1.33 \\
    \cutinhead{Offsets taken from literature}
    3C 33 & S1 & 2.27\pm0.18 ~(2) & Xf & 2.59\pm0.20 & 0.75 &  & 4.86 & 622.00 & 0.14 ~(2) & 0.01 \\
    Pictor A & WHS & 1.00\pm0.15 ~(9) & Xf & 0.69\pm0.10 &  & 0.97\pm0.01 ~(9) & 14.94 & 4810.00 & 76.50 ~(9) & 0.26 \\
    3C 227 & P1/2 & 0.80\pm0.15 ~(10) & Xf & 1.27\pm0.24 &  &  & 8.35 & 41.00 & 1.50 ~(10) & 1.06 \\
     & P3 & 2.30\pm0.15 ~(10) & Xf & 3.66\pm0.24 &  &  & 8.35 & 13.00 & 0.40 ~(10) & 0.89 \\
     & P4 & 0.15\pm0.15 ~(10) & Co-s & 0.24\pm0.24 &  &  & 8.35 & 1.20 & 0.30 ~(10) & 7.25 \\
    3C 273 & A & 0.25\pm0.10 ~(43) & Co-s & 0.68\pm0.27 &  & 0.83\pm0.02 ~(16) &  &  & 46.54 ~(16) & \\
     & B2 & 0.31\pm0.10 ~(43) & Xf & 0.84\pm0.27 &  & 0.97\pm0.03 ~(16) &  &  & 19.98 ~(16) & \\
     & B3 & 0.36\pm0.10 ~(43) & Xf & 0.97\pm0.27 &  & 1.13\pm0.07 ~(16) &  &  & 3.41 ~(16) & \\
     & C1 & 0.14\pm0.10 ~(43) & Co-s & 0.38\pm0.27 &  & 1.07\pm0.06 ~(16) &  &  & 4.85 ~(16) & \\
     & C2 & 0.07\pm0.10 ~(43) & Co-s & 0.18\pm0.27 &  & 0.96\pm0.05 ~(16) &  &  & 6.25 ~(16) & \\
     & H2 & 0.28\pm0.10 ~(43) & Xf & 0.76\pm0.27 &  & 1.27\pm0.12 ~(16) &  &  & 1.30 ~(16) & \\
     & H3 & 0.25\pm0.10 ~(43) & Xf & 0.68\pm0.27 &  & 1.04\pm0.04 ~(16) &  &  & 7.82 ~(16) & \\
     & D1 & 0.18\pm0.10 ~(43) & Co-s & 0.49\pm0.27 &  & 1.02\pm0.05 ~(16) &  &  & 5.16 ~(16) & \\
    3C 327 & S2 & 1.46\pm0.13 ~(10) & Amb & 2.76\pm0.25 &  &  & 8.40 & 99.20 & 0.27 ~(10) & 0.08 \\
     & S1 & 2.24\pm0.17 ~(10) & Xf & 4.23\pm0.32 &  & 0.77\pm0.42  & 8.40 & 41.70 & 0.27 ~(10) & 0.19 \\
    3C 353 & E23 & 1.72\pm0.20 ~(23) & Xf & 1.03\pm0.12 & 0.70\pm 0.03 & 0.81\pm0.29 ~(23) & 1.40 & 11.83 & 0.42 ~(23) & 6.14 \\
     & W47 & 2.21\pm0.20 ~(23) & Xf & 1.32\pm0.12 & 0.63\pm 0.05 &  & 1.40 & 15.58 & 0.31 ~(23) & 3.44 \\
     & E70 & 4.90\pm0.20 ~(23) & Xf & 2.94\pm0.12 & 0.70\pm 0.03 &  & 1.40 & 10.17 & 0.12 ~(23) & 2.04 \\
     & E88 & 6.78\pm0.20 ~(23) & Xf & 4.07\pm0.12 &  & 0.79\pm0.63 ~(23) & 1.40 & 24.82 & 0.24 ~(23) & 1.67 \\
    3C 390.3 & B & 0.40\pm0.15 ~(10) & Xf & 0.43\pm0.16 &  &  & 4.99 & 66.00 & 4.20 ~(10) & 3.09 \\
     & G & 1.00\pm0.20 ~(10) & Xf & 1.08\pm0.22 &  &  & 4.99 & 20.00 & 0.40 ~(10) & 0.97 \\
    Cygnus A & B & 0.15\pm0.15 ~(44) & Co-s & 0.16\pm0.16 &  & 0.75\pm0.19 ~(25) & 8.00 & 2160.00 & 293.10 ~(25) & 4.10 \\
     & A & 0.44\pm0.15 ~(44) & Xf & 0.47\pm0.16 &  & 0.84\pm0.22 ~(25) & 8.00 & 11600.00 & 193.85 ~(25) & 0.51 \\
    4C +74.26 & SHS & 10.00\pm0.15 ~(27) & Xf & 19.00\pm0.28 &  &  & 1.66 & 228.00 & 7.00 ~(27) & 4.48 \\
    3C 445 & SHS & 1.97\pm0.30 ~(30) & Xf & 2.17\pm0.33 &  &  & 8.40 & 81.00 & 0.94 ~(30) & 0.33 \\
\enddata
%\tablecomments{}       
\tablerefs{(1) \citet{2012ApJ...748...81K}. (2) \citet{2007ApJ...659.1008K}. (3) \citet{2004ApJ...612..729H}. (4) \citet{2011ApJ...739...65P}. (5) \citet{2001MNRAS.326.1499H}. (6) \citet{Clautice:2016zai}. (7) \citet{harris2004x}. (8) \citet{hardcastle2001chandra}. (9) \citet{2016MNRAS.455.3526H}. (10) \citet{2007ApJ...669..893H}. (11) \citet{Stanley_2015}. (12) \citet{2006ApJ...641..717S}. (13) \citet{2002ApJ...581..948H}. (14) \citet{2012ApJ...745...84W}. (15) \citet{2018ApJ...860....9M}. (16) \citet{jester2006new}. (17) \citet{Marshall_2002}. (18) \citet{worrall2016x}. (19) \citet{Harris-2017}. (20) \citet{gelbord2005knotty}. (21) \citet{2005MNRAS.360..926W}. (22) \citet{2001ApJ...561L.157B}. (23) \citet{kataoka2008chandra}. (24) \citet{2005ApJ...622..149K}. (25) \citet{wilson2000chandra}. (26) \citet{2008ApJ...684..862S}. (27) \citet{2010MNRAS.404..629E}. (28) \citet{2012ApJ...755..174G}. (29) \citet{2012MNRAS.424.1346W}. (30) \citet{Perlman_2009}. (31) \citet{tavecchio2007chandra}. (32) \citet{2003AA...410..833K}. (33) \citet{siemiginowska2003chandra}. (34) \citet{2012ApJ...750..124S}. (35) \citet{2002ApJ...568..133W}. (36) \citet{jorstad2006x}. (37) \citet{kataoka2003chandra}. (38) \citet{2004ApJ...608..698S}. (39) \citet{2004ApJ...614..615J}. (40) \citet{2011ApJ...729...26M}. (41) \citet{2007ApJ...657..145S}. (42) \citet{Perlman-2011}. (43) \citet{Marchenko_2017}. (44) \citet{pyrzas2015multiwavelength}. (45) \citet{worrall2012jet}.}
%\tablenotetext{b}{The maximum alignment angle is computed using the maximum apparent superluminal motions.}
%% General table references marker
\end{deluxetable*}

%error 0.0615
%A 0.9938542581211589, 0.24709213754524287
%B2 1.9956101843722567, 0.30880878101933945
%B3 2.978928884986831, 0.3562951344185836
%C1 3.999122036874452, 0.13500886638650506
%C2 4.994732221246708, 0.05838524189098687
%D2 5.996488147497801, 0.17662362449551827
%H3 6.973661106233537, 0.2482203028105231
%H2 7.993854258121159, 0.2791079478219227

==> radio_obs.tex <==
    \startlongtable
    \begin{deluxetable*}{lllccl}
        \tablecaption{Details of Radio Observations  \label{table:radio-observations}}
        \tabletypesize{\footnotesize}
        \tablehead{
        \colhead{Name} &
        \colhead{Program}&
        \colhead{Date}&
        \multicolumn{1}{p{1.5cm}}{\centering Frequency\\GHz} &
        \multicolumn{1}{p{2cm}}{\centering Beam \\\as$\times$\as, PA\textdegree}&
        \multicolumn{1}{p{1cm}}{\centering RMS\\$10^{-5}$\nicefrac{Jy}{beam}}
        }
        \tablecolumns{6}
        \startdata
        3C 9 &     15A-357 &  2019 Jun 15 &           14.99 & 0.15$\times$0.12, -55.58 & \phantom{11}0.47 \\
            3C15 &      AB0534 &  1990 May 25 & \phantom{1}8.40 &  0.35$\times$0.26, 51.76 & \phantom{11}2.21 \\
            3C 31 &      AL0405 &  1996 Nov 13 & \phantom{1}8.46 & 0.24$\times$0.22, 167.00 & \phantom{11}1.04 \\
        4C +01.02 &      AR0197 &  1989 Jan 08 & \phantom{1}4.80 &  0.47$\times$0.39, 18.26 & \phantom{1}11.80 \\
            3C 33 &      AR0148 &  1986 Jul 13 & \phantom{1}4.86 & 1.54$\times$1.49, -32.53 &           124.00 \\
            3C 47 &      AB0796 &  1996 Nov 07 & \phantom{1}4.84 &  0.40$\times$0.38, 61.81 & \phantom{11}2.19 \\
    PKS 0144-522 &   ATCA(C890) &  2004 May 08 &           17.73 &   0.40$\times$0.40, 0.00 & \phantom{1}12.10 \\
        4C +35.03 &      AM0221 &  1987 Aug 15 & \phantom{1}4.86 & 0.39$\times$0.36, -20.48 & \phantom{11}5.26 \\
    PKS 0208-512 &  ATCA(C890) &  2002 Feb 01 & \phantom{1}8.64 & 1.33$\times$1.21, -26.06 & \phantom{1}27.40 \\
        3C 66B &      AA0128 &  1991 Aug 19 & \phantom{1}8.21 &   0.24$\times$0.20, 9.80 & \phantom{11}2.66 \\
        4C +28.07 &      AW0482 &  1998 May 24 & \phantom{1}8.47 & 0.23$\times$0.22, -13.17 & \phantom{1}17.80 \\
            3C 78 &      AP0439 &  2003 Sep 06 & \phantom{1}8.46 &  0.25$\times$0.23, -1.58 & \phantom{11}4.06 \\
        3C 83.1 &      GO0001 &  1993 Feb 23 & \phantom{1}4.98 & 1.40$\times$1.20, -84.40 & \phantom{11}4.67 \\
            3C 88 &      AP0077 &  1984 Apr 22 & \phantom{1}4.83 &   4.83$\times$4.29, 5.50 & \phantom{1}24.40 \\
    PKS 0405-12 &      AB0534 &  1990 May 25 & \phantom{1}8.46 &  0.36$\times$0.21, 26.16 & \phantom{11}6.87 \\
        3C 109 &      VG0064 &  1990 Jun 13 & \phantom{1}4.98 &  0.60$\times$0.45, 85.44 & \phantom{11}4.11 \\
    PKS 0413-21 &      AJ0268 &  1999 Jul 02 & \phantom{1}8.46 & 0.51$\times$0.25, -28.45 & \phantom{11}3.09 \\
        3C 123 &      AP0315 &  1995 Aug 07 & \phantom{1}8.44 & 0.22$\times$0.21, -46.55 &           114.00 \\
    PKS 0454-46 &  ATCA(C890) &  2000 Sep 03 & \phantom{1}8.64 &  2.09$\times$0.91, -4.33 &           214.00 \\
    PKS 0605-089 &     16B-332 &  2016 Nov 18 & \phantom{1}9.99 & 0.26$\times$0.16, -22.16 & \phantom{11}1.98 \\
    B2 0738+313 &      AG0589 &  2001 Apr 07 & \phantom{1}4.86 &  1.41$\times$1.22, 68.96 & \phantom{11}2.28 \\
        OJ 248 &      AM0723 &  2003 Aug 28 & \phantom{1}4.86 &  0.39$\times$0.38, 57.67 & \phantom{11}0.56 \\
        4C +29.30 &         VAN &  1982 Feb 07 & \phantom{1}4.80 & 0.55$\times$0.42, -12.34 & \phantom{1}19.80 \\
        3C 207 &     15A-397 &  2015 Aug 08 &           14.99 & 0.13$\times$0.11, -16.08 & \phantom{11}2.22 \\
        OJ 287 &      AS0490 &  1999 Jan 04 & \phantom{1}1.43 & 1.44$\times$1.29, -49.63 & \phantom{1}11.90 \\
        4C +47.29 &      AM0672 &  2000 Nov 05 & \phantom{1}4.86 & 0.63$\times$0.79, -76.76 & \phantom{1}24.00 \\
    PKS 0920-397 &      AH0604 & 1998 May 19  & \phantom{1}8.46 &  0.15$\times$0.13, 68.65 & \phantom{11}5.18 \\
        3C 228 &      AP0331 &  1996 Dec 15 & \phantom{1}8.47 &  0.25$\times$0.22, -2.21 & \phantom{11}4.65 \\
    Q 0957+561 &      AR0247 &  1991 Aug 17 & \phantom{1}8.44 &  0.24$\times$0.21, 79.95 & \phantom{11}1.35 \\
    PKS 1030-357 &  ATCA(C890) &  2004 May 12 &           18.94 &  0.88$\times$0.47, 11.83 & \phantom{11}6.60 \\
        3C 245 &      AK0353 &  1994 Mar 21 & \phantom{1}8.70 & 0.27$\times$0.23, -71.29 & \phantom{1}15.90 \\
    PKS 1045-188 &      BR0044 &  1996 Dec 13 & \phantom{1}8.41 & 0.50$\times$0.25, -17.62 & \phantom{1}17.50 \\
    PKS 1055+201 &      VH0025 &  1986 Jun 02 & \phantom{1}4.98 & 0.75$\times$0.69, -60.50 & \phantom{1}41.30 \\
        3C 254 &      AB0522 &  1989 Feb 01 & \phantom{1}4.86 &  0.49$\times$0.37, 76.70 & \phantom{11}6.76 \\
    PKS 1127-145 &      AC0779 &  2005 May 11 & \phantom{1}8.46 &   0.98$\times$0.69, 6.11 & \phantom{11}6.73 \\
    PKS 1136-135 &      AH0938 &  2003 Nov 08 & \phantom{1}4.86 &  0.57$\times$0.55, 77.00 & \phantom{1}10.30 \\
        3C 263 &      AB0454 &  1987 Jul 12 & \phantom{1}4.86 & 0.53$\times$0.46, 102.00 & \phantom{11}2.53 \\
        3C 265 &      AF0186 &  1990 Sep 16 & \phantom{1}8.44 & 0.92$\times$0.74, -81.86 & \phantom{11}4.21 \\
        4C +49.22 &     16B-189 &  2016 Dec 07 & \phantom{1}4.86 &  0.44$\times$0.39, 19.51 & \phantom{11}0.94 \\
    PKS 1202-262 &      AE0059 &  1988 Oct 30 & \phantom{1}4.86 &   0.50$\times$0.50, 0.00 & \phantom{11}6.06 \\
        3C 270.1 &      AB0796 &  1996 Nov 12 & \phantom{1}8.40 & 0.22$\times$0.22, -41.90 & \phantom{11}1.27 \\
            M84 &      AW0530 &  2008 Nov 18 & \phantom{1}8.40 & 0.42$\times$0.41, 138.00 & \phantom{11}2.28 \\
        4C +21.35 &      AN0122 &  2004 Oct 16 & \phantom{1}8.46 & 0.25$\times$0.22, -57.24 & \phantom{11}9.34 \\
            M87 &     15A-357 &  2015 Aug 01 & \phantom{1}9.99 & 0.26$\times$0.23, -34.67 & \phantom{1}17.60 \\
    PKS 1229-02 &      AK0353 &  1994 Mar 21 & \phantom{1}8.52 & 0.28$\times$0.26, -20.56 & \phantom{11}9.22 \\
        3C 275.1 &      AG0247 &  1987 Sep 14 & \phantom{1}4.86 & 0.42$\times$0.40, -46.06 & \phantom{11}3.81 \\
        3C 277.3 &        VANB &  1981 Mar 18 & \phantom{1}4.87 & 0.44$\times$0.43, -72.87 & \phantom{11}9.80 \\
        4C +52.27 &      AM0723 &  2003 Aug 28 & \phantom{1}4.86 &  0.48$\times$0.38, 54.33 & \phantom{11}3.76 \\
        3C 287.1 &      AS0179 &  1984 Jan 31 & \phantom{1}4.86 & 2.38$\times$1.25, -50.00 & \phantom{1}12.60 \\
    PKS 1335-127 &      AJ0133 &  1986 Mar 21 & \phantom{1}4.86 &   0.52$\times$0.59, 4.54 & \phantom{1}39.20 \\
        4C +19.44 &      S71062 &  2006 Feb 06 & \phantom{1}4.86 &  0.47$\times$0.43, 38.55 & \phantom{11}5.81 \\
        3C 294 &      AM0224 &  1987 Oct 12 & \phantom{1}4.76 &  0.46$\times$0.40, 79.05 & \phantom{11}2.54 \\
        3C 295 &      AC0238 &  1988 Nov 26 & \phantom{1}8.56 & 0.23$\times$0.21, -86.93 & \phantom{11}9.63 \\
        3C 299 &      AP0158 &  1989 Jan 21 & \phantom{1}4.86 &  0.42$\times$0.35, 40.26 & \phantom{1}10.30 \\
    PKS B1421-490 &   ATCA(C890) &  2004 May 08 &           20.16 &   0.79$\times$0.41, 7.24 & \phantom{1}96.00 \\
        3C 303 &      AK0403 &  1995 Jul 27 & \phantom{1}8.44 & 0.41$\times$0.22, -78.30 & \phantom{1}11.70 \\
    PKS 1510-08 &      AO0070 &  1986 May 06 & \phantom{1}4.86 &   0.51$\times$0.39, 7.40 & \phantom{1}11.70 \\
        3C 325 &      AF0213 &  1991 Jul 20 & \phantom{1}4.86 &  0.40$\times$0.38, 32.00 & \phantom{11}2.92 \\
        3C 327 &      AB0534 &  1989 Apr 27 & \phantom{1}8.40 & 0.94$\times$0.90, -27.76 & \phantom{1}10.80 \\
        4C +00.58 &     15A-357 &  2015 Jun 22 & \phantom{1}9.99 &  0.21$\times$0.17, -1.46 & \phantom{11}1.69 \\
        3C 330 &      AF0123 &  1991 Jul 20 & \phantom{1}4.85 &  0.41$\times$0.39, 42.11 & \phantom{11}4.24 \\
        4C +15.55 &      AH0171 &  1985 Jan 02 & \phantom{1}4.80 &  0.48$\times$0.40, 79.87 & \phantom{1}41.70 \\
        3C 346 &      AS0179 &  1985 Mar 03 & \phantom{1}4.86 &   0.36$\times$0.34, 4.00 & \phantom{1}74.40 \\
        3C 345 &      AR0196 &  1989 Jan 08 & \phantom{1}8.44 & 0.23$\times$0.22, -37.60 & \phantom{1}20.90 \\
        4C +69.21 &      AF0310 &  1996 Dec 15 & \phantom{1}8.44 & 0.31$\times$0.20, -20.64 & \phantom{11}8.68 \\
        3C 351  &      UH0001 &  1991 Nov 25 & \phantom{1}8.44 & 1.17$\times$0.81, 110.30 & \phantom{11}3.29 \\
        1800+440 &      AD0337 &  1994 May 04 & \phantom{1}8.44 & 0.24$\times$0.22, -22.61 & \phantom{1}12.90 \\
        4C +56.27 &      AM0672 &  2000 Nov 05 & \phantom{1}4.86 &  0.68$\times$0.38, 79.85 & \phantom{1}13.40 \\
        3C 380 &      AW0101 &  1983 Oct 29 & \phantom{1}4.86 &   0.39$\times$0.37, 7.89 & \phantom{1}94.10 \\
        1849+670 &     16B-386 &  2016 Sep 08 & \phantom{1}9.99 &  0.77$\times$0.55, 54.28 & \phantom{11}0.92 \\
        4C +73.18 &      AE0027 &  1983 Nov 01 & \phantom{1}4.86 & 0.47$\times$0.35, -35.15 & \phantom{1}44.50 \\
        3C 403 &      AB0534 &  1989 Apr 07 & \phantom{1}8.35 & 1.00$\times$0.98, -25.82 & \phantom{11}9.04 \\
    S5 2007+777 &      AH0386 &  1990 Mar 27 & \phantom{1}1.43 & 1.57$\times$0.13, -80.15 & \phantom{1}14.70 \\
    PKS 2101-490 &   ATCA(C890) &  2004 May 08 &           17.73 & 0.92$\times$0.55, 173.50 & \phantom{1}15.70 \\
    PKS 2152-69 & ATCA(C2034) &  2013 Oct 30 &           18.00 &   0.55$\times$0.47, 6.68 & \phantom{11}6.12 \\
        4C +08.64 &      VH0225 &  1986 Jun 01 & \phantom{1}4.80 & 0.45$\times$0.41, -42.75 & \phantom{11}5.17 \\
        4C -03.79 &     16B-121 &  2016 Nov 01 & \phantom{1}6.00 &  0.43$\times$0.27, 34.94 & \phantom{11}1.44 \\
        3C 452 &      AB0534 &  1989 Jul 02 & \phantom{1}8.40 &  0.25$\times$0.25, -0.11 & \phantom{11}9.81 \\
        3C 454.3 &      BR0080 &   2002 Apr 4 & \phantom{1}8.40 & 0.25$\times$0.23, -78.30 & \phantom{11}0.35 \\
    \enddata
    \end{deluxetable*}

==> results.tex <==
\section{Results\label{sec:results}}
Table~\ref{table:offsets} lists the offsets/coincidences in our sample. We've also introduced a nomenclature to denote the nature of an offset and any other miscellaneous atrributes of location of the offset in the jet. Table~\ref{table:offset_nomenclature} provides a summary of this nomenclature. Also, the offsets in each source is qualitatively discussed in Appendix~\ref{sec:notes_on_sources}. The discussion is provided as a figure caption for each source to facilitate easier correspondence of the text with the figure.

%https://asaip.psu.edu/articles/beware-the-kolmogorov-smirnov-test/

The main motive of this study is to infer the presence(or absence therein) of offsets between the radio and X-ray knots in \textit{Chandra} detected X-ray jets. Apart from the previously reported offsets, we find evidence for offsets in several other sources. This suggests that the offsets in X-ray jets are more the norm than an exception. Also, this is contrary to what one would expect from single-zone emission models of the jet. Although, hotspots are not considered a part of the jet\citep{leahy1997study}, we include the offsets found in them for the sake of completeness.

\subsection{Offset source statistics}
\textcolor{blue}{The numbers are subjected to small changes}
There are 91 sources in our sample with atleast one feature that allows us to infer possible offsets between the radio and the X-rays. We find:
\begin{itemize}
    \itemsep -0.5\parsep
    \item clear offsets in knots of 26 sources and a possibility of an offset in 16 other sources.
    \item clear offsets in hotspots of 21 sources and a possibility of an offset in 6 other sources.
    \item coincident knots in 30 sources and atleast 18 of them are superluminal.
    \item coincident hotspots in 19 sources and atleast 7 of them are superluminal.
    %Of them, we find clear(\textcolor{blue}{Is it correct to call the offsets as significant and marginal without any p-value?}) evidence for offsets in knots in 25 sources and a possibility of an offset in 16 other sources. We also find cler evidence for offsets in hotspots in 21 sources and marginal evidence in 9 other sources. In, 27 sources, we find no offsets in atleast one knot and out of them 9 sources also have atleast one knot with an offset. And, 17 of these 27 sources display superluminal motions in their pc scale jets. This suggests that close alignment of the kpc scale jet may play a significant role in \textit{hiding} any existing offsets in them. There are 15 sources with no offset in atleast one hotspot and out them, one source has another hotspot with an offset. Just like in the case of knots, 6 of them have superluminal motions on pc scales. 

\end{itemize}
Fig~\ref{fig:offset_venn_diagrams} shows the information presented above in the form of venn diagrams where each count indicates the number of sources hosting a knot/hotspot with/without an offset.

The absence of offsets in many knots and hotspots of superluminal sources suggests that projection effects may play a  role in \textit{hiding} any possible offsets. But also there is atleast one knot with an offset in 14 superluminal sources. This hiding is probably avoided by a deflection of the kpc-scale jet from pc-scale jet and also from our line of sight as evident from the radio and X-ray images(ex., 605-089 in Fig.~\ref{fig:0605-08_rovx}).
\begin{figure*}
   
    \gridline{
        \boxedfig{images/plots/all_knots_venn-crop.pdf}{0.25\textwidth}{(a) All the sources--knots}
        \boxedfig{images/plots/all_knots_sig_venn-crop.pdf}{0.22\textwidth}{(c) Clear offsets--knots}
        \boxedfig{images/plots/all_knots_mg_venn-crop.pdf}{0.3\textwidth}{(e) Possible offsets--knots}
    }
    \gridline{
        \boxedfig{images/plots/all_hs_venn-crop.pdf}{0.3\textwidth}{(b) All the sources--hotspots}
        \boxedfig{images/plots/all_hs_venn_sig-crop.pdf}{0.3\textwidth}{(d) Clear offsets--hotspots}
        \boxedfig{images/plots/all_hs_venn_mg-crop.pdf}{0.25\textwidth}{(f) Possible offsets--hotspots}
    }
    \caption{Venn diagrams of the counts of sources with offsets/coincidences in knots/hotspots. The top and bottom panels indicate the situation for knots and hotspots respectively. (a) and (b) contain all the sources, (c) and (d) contain only the sources with clear offsets while (e) and (f) contain the sources with possible offsets. \label{fig:offset_venn_diagrams}}


\end{figure*}

\subsection{The 'Xf' offsets} 

The \textit{Xf} offsets, or the offsets where the X-rays peak and decay earlier than the radio,  appear to be more common in our sample than their counterparts, the \textit{Rf} offsets. This is true for all the three classes of sources in our sample: FR I, FR II and Quasars. It suggets that these knots are possibly composed of similar structures that produce X-rays and radio at their upstream and downstream zones respectively. For example, this structure could be a heavy slower moving blob/stationary obstacle surrounded by a faster and lighter outer flow. The first kind of structure was discussed in the context of higher power FR-II jets in section~\ref{sec:vla_sim}. See Fig~\ref{fig:1322-428_rovx} and the references therein for a discussion about the second kind of structure in the context of lower power FR-I sources. In either case, the X-rays and radio may share a commmon workplace initially and their emission zones would diverge later. 

Fig.~\ref{fig:knots_hotspots_parall_coords} shows a categorical parallel coordinate plot of all the offsets/coincidences reported in this work. \textcolor{blue}{Include details on how to read this plot. Also adding a redshift co-ordinate improves the plot}

\begin{figure*}
    %\epsscale{2}
    \gridline{
    %\includegraphics[trim=4cm 1cm 1cm 1cm,clip,width=\textwidth]{images/plots/all_knots_parallel-crop.pdf}
    \boxedfig{images/plots/all_knots_parallel-crop.pdf}{\textwidth}{(a) Knots}
    }
    \gridline{
        \boxedfig{images/plots/all_hotspots_parallel-crop.pdf}{\textwidth}{(b) Hotspots}
    }
    \caption{Categorical parallel coordinates plot for all the offsets found in knots and hotspots. This plot also includes the possible offsets. The first and the second coordinates indicate the class and subclass of the component source. The third coordinate indicates where there are apparent superluminal motions found in the parsec scale jet. The fourth and the final coordinates indicates the type of offset or coincidence. The top and bottom panels represent the knots and hotspots respectively.\label{fig:knots_hotspots_parall_coords}}
\end{figure*}

But, the \textit{Xf} offsets also appear to be common at apparent bends in the jets(indicated with a \textit{+Bnd} in column 3 of Table.~\ref{table:offsets}). Although moving blobs/stationary obstacles can explain the \textit{Xf} offsets, there is no reason to belive that they are also simultaneously responsible for an apparent curvature in the jet. Several authors have proposed that pressure gradients in the intra-cluster medium can deflect the jets that would be accompanied by an internal oblique shock at the bend. Since such shocks could produce X-ray emitting electrons that are expected to have lower radiating times, they might be usually unresolved. \citet{2005MNRAS.360..926W} speculate that a supersonic advance of the jet of \textit{3C346} into the cluster medium after such a bend could generate a weaker shock that produces radio emitting electrons. Since these electons have longer radiating times, they may be detected over a larger volume that produces an \textit{Xf} offset. 

Also, internal shocks associated with bends in the jet produce sub-sonic flows and jets may lose collimation after the bend. \citet{mendoza2001deflection} note that such a loss of collimation can be avoided by means of efficient cooling. They further add that a weaker shock may form after the bend because of a racing condition between the Mach and the bending angles of the jet. This can possibly create an \textit{Xf} offset at a bend in the jet. But, a bend may not always be accompanied by an internal shock depending on the shape of the bend and the radius of the jet\citep{Mendoza_2002}. We refer the reader to \citet{mendoza2001deflection,Mendoza_2002} for a detailed analytical treatment on jet deflection upon its passage through a gas cloud.

Some \textit{Xf} offsets may also be caused by higher density gas clouds that \textit{reflect} the jet(indicated with a \textit{+OutEdg} in column 3 of Table.~\ref{table:offsets}). For example, a high density gas cloud at knot k1 of 3C277.3 reflects the jet from the southeast towards the southwest. In this case, the X-rays are produced by the jet that shock heats and entrains a previously cold optically emitting gas\citep{worrall2016x}; also shown in Fig~\ref{fig:1251+278_rovx}). Here, the term \textit{reflect} is looslely used to denote that the jet gets deflected by the gas without actually passing through it. Fig~\ref{fig:2209+080_rovx} shows a similar outer-edge brightened X-ray emission at an apparent bend to the sothwest in the jet of 2209+080 at knot A. But \textit{HST} 1.6$\mu$m and 600nm observations presented in \citet{breiding2017fermi} reveal no such structures on the outer-edge. So, the jet probably enters knotA from the northeast region presumably in response to an external pressure gradient and the X-rays may not be directly related to the external medium.

\subsection{The 'Rf' offsets}
The \textit{Rf} offsets, or the offsets where the radio peaks and decays early, represent only a minor fraction of the offsets found in our sample. The mechanism that produces this offset is not clearly understood yet. This kind of offset was initially reported in knot J2 of OJ287, a BL Lac object with a Mpc scale jet\citep{2011ApJ...729...26M}. The authors suggested that the knotty structure in the X-rays may be explained by moving blobs that are produced by intermittent activities in the central engine. The turbulence left behind by these moving knots would reaccelarate the electrons to produce the observed radio emission\citep{mizuno2010magnetic}. Although this explained the \textit{Rf} offsets(see Fig.\ref{fig:0851+20}), they favoured an oblique shock model as that also explained an apparent curvature in the jet. Also, knot J4 that lies further down J2, shows an \textit{Xf} offset. This makes it the only jet in our sample to show both kind of offsets.

It is also possible that the radio emitting electrons would advect downstream and lose most of their energy while the jet may have suffered little entrainment from the external medium. In such a case, if the jet is closely aligned to our line of sight, the low energy electrons may produce X-ray emission via IC/CMB downstream of the radio peak. \citet{Meyer_2019} have suggested this mechanism for the production of X-rays in OJ287.

Also, apart from 1030-397, all the \textit{Rf} offsets in the knots are only found in jets with an FR I morphology. In the case of 1030-397, this offset ocurrs at a location where the jet vanishes before it re-emerges at a hotspot(see Fig.\ref{fig:1030-357_rovx}). A similar scenario where the X-ray emission extends slightly further downstream of the radio before the jet vanishes is seen in 1354+195(4C+19.44; Fig.\ref{fig:1354+195_rovx}).

\subsection{Offsets in the hotspots}
A few mechanisms that were suggeted to explain the emission from the hotspots also result in offsets. It is possible that the X-ray hotspot is the present end of the jet while the radio hotspot was its predecessor\citep{scheuer1982}. This transition could be due to a precession or the jet, or a disturbance in the nucleus presumably due to a merger, or any instabilities within the jet itself. This \textit{dentist's drill} model was used to explain the emission from multiple hotspots by \citet{scheuer1982}. Alternately, a spine and sheath configuration can provide an explanation for the offsets\citep{chiaberge2000does}. In this scenario, the spine is a faster and lighter moving material that gets shocked more efficiently than the slower and heavier sheath.  This would produce a bright X-ray emission upstream of the radio hotspot. But there may be a faint X-ray emission that is also coincident with the radio hotspot. It is also  possible that a faster spine in a decelerating jet upscatters the photons from a slower sheath to produce X-ray emission from the hotspots\citep{georganopoulos2003relativistic}. But this would require the jet to be alighed close to the line of sight. 

Sometimes, instead of an offset between X-rays and the radio in a hotspot, there is a double shock structure either in the radio or in the X-rays. For example, there is a double shock structure in the X-rays in the hotspot of 4C+74.26 that are separated by atleast 10kpc\citep{erlund2007luminous}. \citep{erlund2010two} suggest that the structure furthest from the nucleus(outer shock) is located where the jet interacts with the IGM. The inner structure(reverse shock) would be caused by the shocked material that interacts with the jet upstream. In this work, we denote such shock as \textit{Je-HS} where the jet presumably enters the hotspot region. In 4C+74.26, the inner shock dissipates most of the energy of the jet making it the most luminous in the X-rays while the outer shock is fainter and also appears like an arc. 

All these models suggest that the X-rays might peak closer to the core than the radio. But detailed spectral studies and numerical simulations are necessary to correctly infer the acceleration mechanisms in the hotspots. The offsets would also depend strongly on the histories of individual sources. Fig.~\newref{fig:knots_hotspots_parall_coords}{b} shows a parallel coordinate plot for the offsets seen in the hotspots. It is clear from the figure that \textit{Xf} offsets are much more common than the \textit{Rf} kind hotspots similar to what is found in the knots. 

The jets can also flow to a different point on the lobe after an initial impact to create multiple hotspots\citep[e.g.,][]{1986AJ.....92...12L}. In this case, the most compact hotspot would be associated with the present tip of the jet that is commonly referred to as the primary hotspot. \citet{tregillis2001simulating}, in their 3D-MHD simulations, find that the jet and the back-flowing plasma interact to create what they call a ''shock-web complex" that hosts multiple shocks with varying sizes and strengths. They also find that not all of the jet material passes through the terminal shock and that the terminal shock might not always be the strongest one. Also, in their model, the hotspots may not be the regions for particle acceleration rather regions of amplified magnetic fields. This might be the cause of the rare \textit{Rf} offsets in the hotspots found in our sample. \citet{pyrzas2015multiwavelength} find that the peak of  the primary hotspot in the western lobe of \textit{Cygnus A} shift away from the nucleus with increasing frequencies in radio. This is also true in the case of X-rays. They suggest that higher frequency photons are emitted from regions with higher magnetic fields. This, when combined with adiabtic losses of electrons leaving the shock front could lead to the observed offsets.



%Sometimes, the 
%--Refer to the hotspot of 4c+74.21 which shows two shocks displaced by atleast 10kpc--refer to hardcastle 2005(?) for offsets in hotspots--Refer  to the parallel coordinate plot
%\textcolor{blue}{Include histograms of the magnitude of offsets?Talk about how they compare with each other. Also, includes angle estimates from the literature. Compare the ones with the angles to the ones without angles. Also make a comparision with alignment errors in superluminal sources. This might give an idea whether superluminal sources truly hide their offsets or are there any geometric effects of relativity in play}



%\textcolor{blue}{Talk about offsets at bends. Also mention the two sources where the X-rays appear to brighten along the inner edge of the bend. 3C9? Also, thermal emission in 3c277.3 k1, 2209+080}

%\textcolor{blue}{Talk about the the sources where there is still X-ray emission after the radio at an apparent bend in the jet. 1030? 4C+19.44?}

%\textcolor{blue}{Talk about unresolved knots at hotspots and also jets entering the hotspot region. Emphasize that the hotspots are not part of jets?}

%\textcolor{blue}{Talk about the flaring regions in FRIs. Is it possible that the flaring regions in some FR Is are not visible because of finite resolution? If not what is the difference between the ones with and without flaring regions?}

%\textcolor{blue}{Talk about the sources where the X-rays terminate after a bend in the jet. But it could also be the same reason why we don't see knots in the counter jet}

%\textcolor{blue}{Talk about the 'emission from the sheath' in 3C353. TODO: create a good residual image of 3C353}

%\textcolor{blue}{Talk about the rare cases of radio first offsets.}

%\textcolor{blue}{Talk about various explanations that were proposed earlier. Synchrotron cooling. moving blobs(fast and slow)}

%\textcolor{blue}{\textbf{Check the longitudinal profiles in 0637 using different bin-sizes. There is something lurking in there}}





==> vla_simulation.tex <==
\section{What can create offsets in observations?\label{sec:vla_sim}}

As discussed above, there is no universal mechanism that produces an offset. But from an observational point of view, if radio and X-rays come from different zones--even when they are not resolved--can produce a peak-to-peak offset. This section illustrates the emergence of an offset by simulating radio observations of a knot, EJ1, in \textit{3C353}. Figure~\newref{fig:vla_sim_images}{a} shows a 4.8GHz radio image of EJ1 at 0.33\as resolution.
% \newref{fig:vla_sim_images}{b} shows the corresponding X-ray image with radio contours overlaid. 
The X-rays peak upstream of the radio peak in this knot. The jet is inclined to the line of sight at an angle of at least 60deg \citep{swain1998internal}. Therefore the linear size of EJ1 deprojects to atleast 6kpc(scale=0.6 kpc/\as).

\begin{figure*}
    \gridline{
        \boxedfig{images/simulations/3C353_EJ1_r.eps}{0.3\textwidth}{(a) Radio image}
        \boxedfig{images/simulations/3C353_EJ1_rovx.eps}{0.3\textwidth}{(b) X-ray image with radio cotnours}}

        \gridline{
            \boxedfig{images/simulations/0.01_sim.eps}{0.3\textwidth}{(c) Simulation 1}
            \boxedfig{images/simulations/0.006_sim.eps}{0.3\textwidth}{(d) Simulation 2}
            \boxedfig{images/simulations/0.003_sim.eps}{0.3\textwidth}{(e) Simulation 3}}
    \gridline{
   \boxedfig{images/simulations/0.01_skymodel.eps}{0.3\textwidth}{(f) Source 1}
   \boxedfig{images/simulations/0.006_skymodel.eps}{0.3\textwidth}{(g) Source 2}
   \boxedfig{images/simulations/0.003_skymodel.eps}{0.3\textwidth}{(h) Source 3}}
   
   
    \caption{VLA X(8.4GHz) band B config simulations of the knot EJ1 in \textit{3C353}. (a) shows the radio knot EJ1 in \textit{3C353} while (b) shows the corresponding X-ray knot with radio contours overlaid on it.  The 'X' points to the location of the X-ray peak , and the dashed arrow follows the direction of the jet. The middle panel shows the simulated images of EJ1 at different redshifts. The bottom panel shows the knots with contours from their corresponding simulated observations\label{fig:vla_sim_images}}
\end{figure*}

%Now we ferry this knot to three different redshifts: where the angular scales are about 2.5, 4, 8.3 kpc/\as. The sizes of the knot 
Now we ferry this knot to three different redshifts while keeping the flux constant. The first column of Table.~\ref{table:vla_sim} gives the angular scale at each redshift; the second column gives the corresponding angular size of EJ1. The third column provides an example source that lies at a similar redshift.

%become 2.4\as, 1.5\as, 0.7\as in the same order. For example, \textit{4C+13.41}, \textit{3C273} and \textit{PKS1127-145} in the same order lie at similar redshifts of the considered angular scales. 
We simulate a VLA observation in the X-band B-configuration (\siml0.7\as resolution) at each position  using \textit{simobserve} and \textit{simanalyze} tasks in \textit{CASA}.
 \begin{deluxetable}{ccc}
    %\tabletypesize{\scriptsize}
    \tablecaption{Details of the simulations of VLA observations\label{table:vla_sim}}
\tablehead{
    \colhead{Angular scale (kpc/\as)} & \colhead{Knot's size (\as)} & \colhead{Nearby source}
    %\colhead{scale (kpc/\as)} & \colhead{size (\as)} & \colhead{source}
}
\startdata
2.5 & 2.4 & \textit{4C+13.41}\\
4 & 1.5 & \textit{3C273}\\
8.3 & 0.7 & \textit{PKS1127-145}
\enddata
\end{deluxetable}
\placetable{table:vla_sim}
The middle panel of Fig.~\ref{fig:vla_sim_images} shows the simulated images while their contours are overlaid on the observed sources in the bottom panel.  
The telescope resolves the knot at first and second redshifts and it doesn't at the third. But in all the three simulations, the obtained peak doesn't match the actual radio peak; it lies close to the weighted centroid of the brightness distribution. And the radio peaks offset the X-rays by \siml0.2\as. We can, for example, speculate that this is the cause for the offset in knot B of \textit{PKS1127-145} using simulation 3, both which lie at similar redshifts. It is plausible that the jet makes an angle of 15deg to our line of sight \citep{2007ApJ...657..145S}. If the actual size of the knot was about 20kpc, the projected size would equal the size of EJ1. And if X-rays were to peak at the same location as in EJ1, the offset found in the third simulation can match the observed offset of \siml0.2\as \citep{2007ApJ...657..145S}.

These simulations are simplistic for they overlook many physical and observational effects. All the radio knots, at least in high power jets, may not only exist in the sheath. There can be a change of flux with redshift or frequency. The observations can include thermal noise, atmospheric contamination, etc., The jet may be inclined close to our line of sight and the offset may not be visible because of finite resolution. But this exercise suggests that if the radio and X-rays are coming from different zones in the jet, it can induce a peak-to-peak \textit{offset}. That means, in a sense, if either one of X-ray or radio decays earlier than the other one, it produces an offset. But, they may share a common working surface. For example, a possible shock front in the upstream edge of radio knot EJ1. Also, if such a shock front is sufficiently brighter than the rest of the knot, the peak of the unresolved knot can lie close to the X-ray peak. And an offset may not be seen in such cases.



==> xray_first_hotspots.tex <==
\begin{deluxetable}{ccc}
\tablewidth{\textwidth}
\tablecaption{List of sources with X-ray first hotspot(s)\label{table:hs_xray_first_src_list}}
\startdata
\\[0.5em]
3C6.1&3C111&Pictor A\\
3C227&3C452
\enddata
\end{deluxetable}

\begin{deluxetable}{ccc}
\tablewidth{\textwidth}
\tablecaption{List of sources with co-spatial hotspot(s) in radio and X-rays\label{table:cospatial_hs_src_list}}
\startdata
\\[0.5em]
3C6.1&3C47&PKS0405-12&3C109\\
3C123
\enddata
\end{deluxetable}

==> xray_obs.tex <==
\startlongtable
    \begin{deluxetable*}{l>{\raggedright}p{3cm}clc}
      %\centerwidetable
      \tablecaption{Details of \textit{Chandra} X-ray Observations \label{table:xray-observations}}
      \tabletypesize{\footnotesize}
      \tablewidth{0pt}
      \tablehead{
        \colhead{Name} &
        \multicolumn{1}{p{3cm}}{\centering Chandra\\ObsIDs} &
        \multicolumn{1}{p{2cm}}{\centering Effective\\exposure\textsuperscript{a} (ks)} &
        \colhead{Modes\textsuperscript{b}}&
        \colhead{\nicefrac{counts}{s}\textsuperscript{c}}
        %\multicolumn{1}{p{2cm}}{\centering X-ray image\\scale}&
      }
      \tablecolumns{5}
      \startdata
      3C 9 &                          1595, 17088, 18700-1 & \phantom{1}89.00 & F, V & 0.021 \\
      3C15 &                                              17128 &           116.34 &    V & 0.045 \\
     3C 31 &                                               2147 & \phantom{1}44.00 &    F & 0.027 \\
 4C +01.02 &                                 9281, 10380, 10799 & \phantom{1}70.30 &    V & 0.163 \\
     3C 33 &                                         6910, 7200 & \phantom{1}36.40 &    F & 0.068 \\
     3C 47 &                                               2129 & \phantom{1}34.70 &    F & 0.222 \\
PKS 0144-522 &                                              10366 & \phantom{11}5.41 &    V & 0.091 \\
 4C +35.03 &                                                856 & \phantom{11}8.20 &    V & 0.020 \\
PKS 0208-512 &                                         3108, 4813 & \phantom{1}50.80 & F, V & 0.286 \\
    3C 66B &                                                828 & \phantom{1}44.00 &    F & 0.045 \\
 4C +28.07 &                                        4898, 17089 & \phantom{1}43.40 & V, V & 0.211 \\
     3C 78 &                                               4157 & \phantom{1}47.41 &    V & 0.444 \\
   3C 83.1 &                                               3237 & \phantom{1}71.38 &    V & 0.011 \\
     3C 88 &                                11751, 11977, 12007 & \phantom{1}97.70 &    V & 0.016 \\
PKS 0405-12 &                                               2131 & \phantom{11}6.30 &    F & 0.036 \\
PKS 0413-21 &                                               3117 & \phantom{11}4.37 &    F & 0.075 \\
    3C 123 &                                                829 & \phantom{1}27.82 &    F & 0.015 \\
PKS 0454-46 &                                               4893 & \phantom{11}5.80 &    F & 0.363 \\
PKS 0605-089 &                                 2132, 11431, 12056 & \phantom{1}66.60 &    F & 0.255 \\
PKS 0637-752 &                  19692, 20864-7 &           108.56 &    F & 0.592 \\
B2 0738+313 &                                                377 & \phantom{1}26.00 &    F & 0.141 \\
    OJ 248 &                                               3047 & \phantom{1}17.50 &    F & 0.351 \\
 4C +29.30 &                   2135, 11688-9, 12106, 12119 &           222.99 & F, V & 0.024 \\
    3C 207 &                                               2130 & \phantom{1}14.33 &    F & 0.178 \\
    OJ 287 &                                               9182 & \phantom{1}42.20 &    F & 0.446 \\
PKS 0920-397 &                       3114, 5732, 7220, 7221, 7223 & \phantom{1}83.06 &    F & 0.137 \\
    3C 228 &                                         2095, 2453 & \phantom{1}22.34 &    F & 0.025 \\
Q 0957+561 & 362, 2038, 12076, 12077-87 & \phantom{1}78.75 & F, V & 0.170 \\
PKS 1030-357 &                                         3115, 5730 & \phantom{1}31.30 &    F & 0.063 \\
PKS 1045-188 &                                        9280, 15037 & \phantom{1}55.00 &    V & 0.164 \\
PKS 1055+201 &                             4889, 5733, 7795-6 &           230.63 & F, V & 0.264 \\
    3C 254 &                                               2209 & \phantom{1}24.50 &    V & 0.188 \\
PKS 1127-145 &                                          866, 5708 &           126.00 &    V & 0.572 \\
PKS 1136-135 &                                         2138, 3973 & \phantom{1}74.70 & F, V & 0.284 \\
    3C 263 &                                               2126 & \phantom{1}24.30 &    F & 0.197 \\
    3C 265 &                                               2984 & \phantom{1}41.20 &    F & 0.006 \\
 4C +49.22 &                                         2139, 3974 & \phantom{1}63.19 & F, V & 0.593 \\
PKS 1202-262 &                                         3118, 4812 & \phantom{1}38.80 & F, V & 0.193 \\
  3C 270.1 &                                        9255, 13906 & \phantom{1}97.31 &    F & 0.085 \\
       M84 &                         803, 963, 1619, 5908, 6131 &           120.40 &    F & 0.033 \\
 4C +21.35 &                                               3049 & \phantom{1}17.40 &    F & 0.447 \\
       M87 &                                               2707 & \phantom{1}88.43 &    F & 0.086 \\
PKS 1229-02 &                                         3118, 4812 & \phantom{1}38.80 & F, V & 0.191 \\
  3C 275.1 &                                               2096 & \phantom{1}20.90 &    F & 0.174 \\
  3C 277.3 &                                              11391 & \phantom{1}23.20 &    V & 0.057 \\
 4C +52.27 &                                               3050 & \phantom{1}11.40 &    F & 0.149 \\
  3C 287.1 &                                               9309 & \phantom{11}7.70 &    V & 0.222 \\
PKS 1335-127 &                                               9282 & \phantom{11}9.87 &    V & 0.378 \\
 4C +19.44 &                 2140, 6903-4, \mbox{7302-3} &           143.66 &    F & 0.594 \\
    3C 294 &                                               3207 &           112.52 &    V & 0.001 \\
    3C 295 &                                                578 & \phantom{1}14.50 &    F & 0.015 \\
    3C 299 &                                       10381, 12019 & \phantom{1}45.40 &    V & 0.002 \\
PKS B1421-490 &                                         4895, 5729 & \phantom{1}50.68 &    F & 0.042 \\
    3C 303 &                                               1623 & \phantom{1}13.90 &    V & 0.199 \\
PKS 1510-08 &                                        2141, 11432 & \phantom{1}52.20 &    F & 0.623 \\
    3C 325 &                                         4818, 6267 & \phantom{1}54.20 &    V & 0.012 \\
    3C 327 &                                               6841 & \phantom{1}38.60 &    V & 0.021 \\
 4C +00.58 &                                        9274, 10304 & \phantom{1}99.30 &    F & 0.011 \\
    3C 330 &                                               2127 & \phantom{1}40.80 &    F & 0.004 \\
 4C +15.55 &                                               3229 & \phantom{1}48.80 &    V & 0.033 \\
    3C 346 &                                               3129 & \phantom{1}38.90 &    F & 0.073 \\
    3C 345 &                                 2143, 10379, 12011 & \phantom{1}62.30 & F, V & 0.546 \\
 4C +69.21 &                          2142, 17090, 18762-3 & \phantom{1}68.18 & F, V & 0.087 \\
   3C 351  &                                          435, 2128 & \phantom{1}47.90 & V, F & 0.168 \\
  1800+440 &                                               9286 & \phantom{11}8.20 &    V & 0.176 \\
 4C +56.27 &                                              10369 & \phantom{11}5.11 &    V & 0.518 \\
    3C 380 &                                               3124 & \phantom{11}5.00 &    F & 0.515 \\
  1849+670 &                                 9291, 15038, 16322 & \phantom{1}78.69 &    V & 0.301 \\
 4C +73.18 &                          2145, 13393, 14408, 17091 & \phantom{1}58.60 & F, V & 0.534 \\
    3C 403 &                                               2968 & \phantom{1}25.50 &    F & 0.043 \\
S5 2007+777 &                                               5709 & \phantom{1}28.60 &    F & 0.231 \\
PKS 2101-490 &                                         3126, 5731 & \phantom{1}39.30 &    F & 0.085 \\
PKS 2152-69 &                                 1627, 16083-4 &           175.80 &    V & 0.192 \\
 4C +08.64 &                                               3051 & \phantom{1}16.90 &    F & 0.271 \\
 4C -03.79 &                                        9285, 15039 & \phantom{1}56.40 &    V & 0.155 \\
    3C 452 &                                               2195 & \phantom{1}72.90 &    F & 0.032 \\
  3C 454.3 &                                               4843 & \phantom{1}17.70 &    F & 1.150 \\
             \enddata
             \tablenotetext{a}{After background flare removal, if any.}
             \tablenotetext{b}{The observation mode for each obsID where F=FAINT, V=VFAINT. A single value is provided if all the current and subsequent obsIDs have the same mode.  }
             \tablenotetext{c}{Average of the count rate from each epoch.}
            \end{deluxetable*}
    
